Formal Poincare'-Dulac renormalization for holomorphic germs

In this revised version, applying a general renormalization procedure for formal self-maps, producing a formal normal form simpler than the classical Poincar\'e-Dulac normal form, we shall give a complete list of normal forms for bi-dimensional superattracting germs with non-vanishing quadratic term; in most cases, our normal forms will be the simplest possible ones (in the sense of Wang, Zheng and Peng). We shall also discuss a few examples of renormalization of germs tangent to the identity, revealing interesting second-order resonance phenomena.

==> 0264396.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% These are the macroes
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\ifsect\newif\iffinal
\secttrue\finalfalse
\def\thm #1: #2{\medbreak\noindent{\bf #1:}\if(#2\thmp\else\thmn#2\fi}
\def\thmp #1) { (#1)\thmn{}}
\def\thmn#1#2\par{\enspace{\sl #1#2}\par
        \ifdim\lastskip<\medskipamount \removelastskip\penalty 55\medskip\fi}
\def\square{{\msam\char"03}}
\def\qedn{\thinspace\null\nobreak\hfill\square\par\medbreak}
\def\pf{\ifdim\lastskip<\smallskipamount \removelastskip\smallskip\fi
        \noindent{\sl Proof\/}:\enspace}
\def\itm#1{\item{\rm #1}\ignorespaces}
\let\smbar=\bar
\def\bar#1{\overline{#1}}
%
%\input pdfcolor
%
%\input boxedeps
%\input boxedeps.cfg
%\HideDisplacementBoxes
%%
%\def\Figuraeps #1 (#2){\message{Figura #1}
%	\midinsert      
%	\centerline{\BoxedEPSF{#2.eps}}
%	\bigskip
%	\centerline{\bf Figure~#1}
%	\endinsert}
%%
%\def\Figurascaledeps #1 (#2)(#3){\message{Figura #1}
%	\midinsert      
%	\centerline{\BoxedEPSF{#2.eps scaled #3}}
%	\bigskip
%	\centerline{\bf Figure~#1}
%	\endinsert}
%
%
\newcount\parano
\newcount\eqnumbo
\newcount\thmno
\newcount\versiono
\newcount\remno
\newbox\notaautore
\def\neweqt#1$${\xdef #1{(\number\parano.\number\eqnumbo)}
    \eqno #1$$
    \global \advance \eqnumbo by 1}
\def\newrem #1\par{\global \advance \remno by 1
    \medbreak
{\bf Remark \the\parano.\the\remno:}\enspace #1\par
\ifdim\lastskip<\medskipamount \removelastskip\penalty 55\medskip\fi}
\def\newthmt#1 #2: #3{\xdef #2{\number\parano.\number\thmno}
    \global \advance \thmno by 1
    \medbreak\noindent
    {\bf #1 #2:}\if(#3\thmp\else\thmn#3\fi}
\def\neweqf#1$${\xdef #1{(\number\eqnumbo)}
    \eqno #1$$
    \global \advance \eqnumbo by 1}
\def\newthmf#1 #2: #3{\xdef #2{\number\thmno}
    \global \advance \thmno by 1
    \medbreak\noindent
    {\bf #1 #2:}\if(#3\thmp\else\thmn#3\fi}
\def\forclose#1{\hfil\llap{$#1$}\hfilneg}
\def\newforclose#1{
	\ifsect\xdef #1{(\number\parano.\number\eqnumbo)}\else
	\xdef #1{(\number\eqnumbo)}\fi
	\hfil\llap{$#1$}\hfilneg
	\global \advance \eqnumbo by 1
	\iffinal\else\rsimb#1\fi}
\def\forevery#1#2$${\displaylines{\let\eqno=\forclose
        \let\neweq=\newforclose\hfilneg\rlap{$\qquad\quad\forall#1$}\hfil#2\cr}$$}
%
\def\noNota #1\par{}
\def\today{\ifcase\month\or
   January\or February\or March\or April\or May\or June\or July\or August\or
   September\or October\or November\or December\fi
   \space\number\year}
\def\inizia{\ifsect\let\neweq=\neweqt\else\let\neweq=\neweqf\fi
\ifsect\let\newthm=\newthmt\else\let\newthm=\newthmf\fi}
\def\bititolo{\empty}
\gdef\begin #1 #2\par{\xdef\titolo{#2}
\ifsect\let\neweq=\neweqt\else\let\neweq=\neweqf\fi
\ifsect\let\newthm=\newthmt\else\let\newthm=\newthmf\fi
\iffinal\let\Nota=\noNota\fi
\centerline{\titlefont\titolo}
\if\bititolo\empty\else\medskip\centerline{\titlefont\bititolo}
\xdef\titolo{\titolo\ \bititolo}\fi
\bigskip
\centerline{\bigfont
\autore \ifvoid\notaautore\else\footnote{${}^1$}{\unhbox\notaautore}\fi}
\bigskip\if\istituto!\centerline{\today}\else
\centerline{\istituto}
\centerline{\indirizzo}
%\centerline{E-mail: \email}
\medskip
\centerline{#1\ \anno}\fi
\bigskip\bigskip
\ifsect\else\global\thmno=1\global\eqnumbo=1\fi}
\def\anno{2010}
%
\def\raggedleft{\leftskip2cm plus1fill \spaceskip.3333em \xspaceskip.5em
\parindent=0pt\relax}
\def\dafare{\par\smallskip\begingroup\Bittersweet\raggedleft}
\def\enddafare{\par\endgroup\pdfsetcolor{0. 0. 0. 1.}\smallbreak}
\def\danota{\par\begingroup\ForestGreen\raggedleft}
\let\enddanota=\enddafare
\def\datogliere{\par\begingroup\Blue\raggedleft}
\let\enddatogliere=\enddafare
%
\font\titlefont=cmssbx10 scaled \magstep1
\font\bigfont=cmr12
\font\eightrm=cmr8
\font\sc=cmcsc10
\font\bbr=msbm10
\font\sbbr=msbm7
\font\ssbbr=msbm5
\font\msam=msam10
\font\gto=eufm10
\font\bfm=cmmib10
\font\bfsy=cmbsy10
\def\ca #1{{\cal #1}}
\def\gt #1{\hbox{\gto #1}}
\nopagenumbers
\binoppenalty=10000
\relpenalty=10000
\newfam\amsfam
\textfont\amsfam=\bbr \scriptfont\amsfam=\sbbr \scriptscriptfont\amsfam=\ssbbr
\newfam\boldifam
\textfont\boldifam=\bfm
%
\let\de=\partial
\let\eps=\varepsilon
\let\phe=\varphi
\def\Hol{\mathop{\rm Hol}\nolimits}
\def\Aut{\mathop{\rm Aut}\nolimits}
\def\Hom{\mathop{\rm Hom}\nolimits}
\def\Fix{\mathop{\rm Fix}\nolimits}
\def\Sing{\mathop{\rm Sing}\nolimits}
\def\End{\mathop{\rm End}\nolimits}
\def\Ker{\mathop{\rm Ker}\nolimits}
\def\Res{\mathop{\rm Res}\nolimits}
\def\Re{\mathop{\rm Re}\nolimits}
\def\Im{\mathop{\rm Im}\nolimits}
\def\sp{\mathop{\rm sp}\nolimits}
\def\id{\mathop{\rm id}\nolimits}
\def\rk{\mathop{\rm rk}\nolimits}
\def\ord{\mathop{\rm ord}\nolimits}
\def\diag{\mathop{\rm diag}\nolimits}
\def\Jac{\mathop{\rm Jac}\nolimits}
\def\Span#1{\mathop{\rm Span}\nolimits\left(#1\right)}
\def\bigoperp{\mathbin{\hbox{$\bigcirc\kern-11.8pt\perp$}}}
\def\hz{\hat{z}}
\def\hf{\hat{f}}
\def\hg{\hat{g}}
\def\ha{\hat{a}}
\def\hb{\hat{b}}
\mathchardef\void="083F
\mathchardef\ellb="0960
\mathchardef\taub="091C
\def\C{{\mathchoice{\hbox{\bbr C}}{\hbox{\bbr C}}{\hbox{\sbbr C}}
{\hbox{\sbbr C}}}}
\def\R{{\mathchoice{\hbox{\bbr R}}{\hbox{\bbr R}}{\hbox{\sbbr R}}
{\hbox{\sbbr R}}}}
\def\N{{\mathchoice{\hbox{\bbr N}}{\hbox{\bbr N}}{\hbox{\sbbr N}}
{\hbox{\sbbr N}}}}
\def\P{{\mathchoice{\hbox{\bbr P}}{\hbox{\bbr P}}{\hbox{\sbbr P}}
{\hbox{\sbbr P}}}}
\def\Q{{\mathchoice{\hbox{\bbr Q}}{\hbox{\bbr Q}}{\hbox{\sbbr Q}}
{\hbox{\sbbr Q}}}}
\def\Z{{\mathchoice{\hbox{\bbr Z}}{\hbox{\bbr Z}}{\hbox{\sbbr Z}}
{\hbox{\sbbr Z}}}}
\def\Downarrow{\Big\downarrow}
\def\mapright#1{\smash{\mathop{\longrightarrow}\limits^{#1}}}
\def\rmapdown#1{\Big\downarrow\rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}
\def\lmapdown#1{\llap{$\vcenter{\hbox{$\scriptstyle#1$}}$}\Big\downarrow}
\def\arrowbar{\top}
\def\Downmapsto{\vcenter{\offinterlineskip\halign{\hfil$##$\hfil\cr
\arrowbar\cr\Downarrow\cr}}}
%
\newcount\notitle
\notitle=1
\headline={\ifodd\pageno\rhead\else\lhead\fi}
\def\rhead{\ifnum\pageno=\notitle\iffinal\hfill\else\hfill\tt Version
\the\versiono; \the\day/\the\month/\the\year\fi\else\hfill\eightrm\titolo\hfill
\folio\fi}
\def\lhead{\ifnum\pageno=\notitle\hfill\else\eightrm\folio\hfill\autore\hfill
\fi}
%
\newbox\bibliobox
\def\setref #1{\setbox\bibliobox=\hbox{[#1]\enspace}
    \parindent=\wd\bibliobox}
\def\biblap#1{\noindent\hang\rlap{[#1]\enspace}\indent\ignorespaces}
\def\art#1 #2: #3! #4! #5 #6 #7-#8 \par{\biblap{#1}#2: {\sl #3\/}.
    #4 {\bf #5} (#6)\if.#7\else, \hbox{#7--#8}\fi.\par\smallskip}
\def\book#1 #2: #3! #4 \par{\biblap{#1}#2: {\bf #3.} #4.\par\smallskip}
\def\coll#1 #2: #3! #4! #5 \par{\biblap{#1}#2: {\sl #3\/}. In {\bf #4,}
#5.\par\smallskip}
\def\pre#1 #2: #3! #4! #5 \par{\biblap{#1}#2: {\sl #3\/}. #4, #5.\par\smallskip}
%
%\def\Bittersweet{\pdfsetcolor{0. 0.75 1. 0.24}} % PANTONE 167
%\def\Black{\pdfsetcolor{0. 0. 0. 1.}} % PANTONE 167
\def\raggedleft{\leftskip2cm plus1fill \spaceskip.3333em \xspaceskip.5em
\parindent=0pt\relax}
\def\Nota #1\par{\medbreak\begingroup\Bittersweet\raggedleft
#1\par\endgroup\Black
\ifdim\lastskip<\medskipamount \removelastskip\penalty 55\medskip\fi}
%
\def\ragcn{\leftskip=0pt plus 4em \rightskip=\leftskip
\parfillskip=0pt \spaceskip=0.3333em \xspaceskip=0.5em
\pretolerance=9999 \tolerance=9999 \hyphenpenalty=9999
\exhyphenpenalty=9999}
%
\newcount\defno
\def\smallsect #1. #2\par{\bigbreak\noindent{\bf #1.}\enspace{\bf #2}\par
    \global\parano=#1\global\eqnumbo=1\global\thmno=1\global\defno=0\global\remno=0
    \nobreak\smallskip\nobreak\noindent\message{#2}}
\def\newdef #1\par{\global \advance \defno by 1
    \medbreak
{\bf Definition \the\parano.\the\defno:}\enspace #1\par
\ifdim\lastskip<\medskipamount \removelastskip\penalty 55\medskip\fi}
\finalfalse
\versiono=2
%

\magnification\magstephalf

%%%% Abbreviazioni
\let\no=\noindent
\let\bi=\bigskip
\let\me=\medskip
\let\sm=\smallskip
\let\ce=\centerline
\let\ri=\rightline
\let\te=\textstyle
\let\gd=\goodbreak
\let\io=\infty
\def\qqquad{\quad\qquad}
\finaltrue
%
\def\autore{Marco Abate${}^1$, Jasmin Raissy${}^2$\footnote{${}^*$}{\eightrm Partially supported by FSE, Regione Lombardia.}}
\def\indirizzo{\vbox{\hfill${}^2$Dipartimento di Matematica e Applicazioni, Universit\`a degli Studi
di Milano Bicocca,\hfill\break\null\hfill Via Cozzi 53, 20125 Milano, Italy.
E-mail: jasmin.raissy@unimib.it\hfill\null}}
\def\istituto{\vbox{\hfill${}^1$Dipartimento di Matematica, Universit\`a
di Pisa,\hfill\break\null\hfill Largo Pontecorvo 5, 56127 Pisa,
Italy. E-mail: abate@dm.unipi.it\hfill\null\vskip5pt}}
\def\email{}
%
\begin {August} Formal Poincar\'e-Dulac renormalization for holomorphic germs

{{\narrower{\sc Abstract.}  We describe a general renormalization procedure for germs of holomorphic (or even formal) self-maps, producing a formal normal form simpler than the classical 
Poincar\'e-Dulac normal form. As an example of application of our method we provide a complete 
list of normal forms for quadratic bi-dimensional superattracting germs, that could not be
simplified using the classical Poincar\'e-Dulac normalization only. Finally, we also discuss a few
examples of renormalization of germs tangent to the identity, revealing interesting
second-order resonance phenomena.\par
}}
\smallsect 0. Introduction

\def\autore{Marco Abate and
Jasmin Raissy}

In the study of a class of holomorphic dynamical systems, an 
important goal often is the classification under topological, holomorphic or formal 
conjugation. In particular, for each dynamical system in the class one would like to have a 
definite way of choosing a (hopefully simpler, possibly unique) representative in the same
conjugacy class; a {\sl normal form} of the original dynamical system.

The most famous kind of normal form for local holomorphic dynamical systems
(i.e., germs of holomorphic vector fields at a singular point, or germs of 
holomorphic self-maps with a fixed point) is the {\sl Poincar\'e-Dulac normal form}
with respect to formal conjugation, 
introduced at the end of the nineteenth century. Let us recall very quickly its definition,
at least in the setting we are interested here, that is of germs of self-maps with a fixed point,
that we can assume to be the origin in $\C^n$. Moreover, since we are discussing formal
normal forms,
we shall work with formal transformations of $\C^n$, that is $n$-tuples of power series, without 
discussing here convergence issues.

So let $F\in\widehat\ca O^n$ be a formal transformation in $n$ complex variables,
where $\widehat\ca O^n$ denotes the space of $n$-tuples of
power series in $n$ variables fixing the origin (that is, with vanishing constant term),
and let $\Lambda$ denote the (not necessarily invertible) linear term of~$F$. For simplicity,
given a linear map $\Lambda\in M_{n,n}(\C)$ we shall denote by $\widehat\ca O^n_\Lambda$ 
the set of formal transformations in $\widehat\ca O^n$ with $\Lambda$ as
linear part.
If $\lambda_1,\ldots,\lambda_n$
are the eigenvalues of~$\Lambda$, we shall say that a multi-index $Q=(q_1,\ldots,q_n)\in\N^n$
with $q_1+\cdots+q_n\ge 2$ is {\sl $\Lambda$-resonant} if there is $j\in\{1,\ldots,n\}$
such that $\lambda_1^{q_1}\cdots\lambda_n^{q_n}=\lambda_j$. If this happens, we shall
say that the monomial $z_1^{q_1}\cdots z_n^{q_n}e_j$ is {\sl $\Lambda$-resonant,} where
$\{e_1,\ldots, e_n\}$ is the canonical basis of $\C^n$. Then (for a proof see, e.g., [Ar]):

\newthm Theorem \PD: (Poincar\'e 1893, Dulac 1904) Let $F\in\widehat\ca O^n_\Lambda$ be a formal transformation in $n$ complex variables fixing the origin, with $\Lambda$ in Jordan normal form. Then there exists an invertible
formal transformation $\Phi\in\widehat\ca O^n_I$ with identity linear part such that
$G=\Phi^{-1}\circ F\circ\Phi$ contains only $\Lambda$-resonant monomials.

The formal transformation $G$ is a {\sl Poincar\'e-Dulac normal form} of~$F$; notice that, since
$\Phi\in\widehat\ca O^n_I$, the linear part of $G$ is still~$\Lambda$. More generally,
we shall say that a $G\in\widehat\ca O^n_\Lambda$ is {\sl in Poincar\'e-Dulac normal form}
if $G$ contains only $\Lambda$-resonant monomials.

The importance of this result cannot be underestimated, and it has been applied uncountably
many times; however it has some limitations. For instance, if $\Lambda=O$ or $\Lambda=I$
then {\it all} monomials are resonant; and thus in these cases the Poincar\'e-Dulac normal form
reduces to the original map. More generally, as we shall try and explain below, even when 
the Poincar\'e-Dulac normal form is a simplification of the original germ, it is still possible to further simplify the germ 
(to {\sl renormalize} it) by applying invertible transformations preserving the property of being in 
Poincar\'e-Dulac normal form.  

This idea of renormalizing Poincar\'e-Dulac normal forms is not new in the context of vector 
fields, where it also has been studied the concept of hypernormal 
forms, obtained (roughly speaking) by renormalizing infinitely many times; see, e.g., 
[AFGG, B, BS, G, KOW, LS, Mu1, Mu2] and references therein.
On the other hand, this idea has not yet been fully exploited in the context of
self-maps (one of the few exceptions is [AT1], where it is applied to
a particular class of self-maps with identity linear part). The aim of this paper is to
describe in general the renormalization procedure for formal transformations in several
complex variables, following the general ideas (but with significantly different details)
of the vector field case. We shall then apply this procedure to the case of superattracting
(i.e., with $\Lambda=O$) 2-dimensional formal transformations, case that has no analogue
in the vector field setting. We shall also discuss a few interesting examples with $\Lambda=I$,
in particularly showing the appearance of second-order resonance phenomena.

We conclude this introduction by roughly describing the renormalization procedure. To explain
it better, let us first recast the Poincar\'e-Dulac normalization in slightly different terms
(see also [R\"u]). For each $\nu\ge 2$ let $\ca H^\nu$ denote the space of $n$-tuples of
homogeneous polynomials in $n$ variables of degree~$\nu$. Then
every $F\in\widehat\ca O^n_\Lambda$ admits a {\sl homogeneous expansion}
$$
F=\Lambda+\sum_{\nu\ge 2} F_\nu\;,
$$
where $F_\nu\in\ca H^\nu$ is the {\sl $\nu$-homogeneous term} of~$F$. We shall also use
the notation $\{G\}_\nu$ to denote the $\nu$-homogeneous term of a formal transformation~$G$.

If
$$
\Phi=I+\sum_{\nu\ge 2} H_\nu
$$
is the homogeneous expansion of an invertible formal transformation $\Phi\in\widehat\ca O^n_I$,
then it turns out that there exists a linear operator $L_\Lambda\colon\widehat\ca O^n\to
\widehat\ca O^n$, given by
$$
L_\Lambda(H)=H\circ\Lambda-\Lambda H\;,
$$
sending each $\ca H^\nu$ into itself and such that
$$
\{\Phi^{-1}\circ F\circ\Phi\}_\nu=F_\nu-L_\Lambda(H_\nu)+R_\nu
$$
for all $\nu\ge 2$, where $R_\nu$ is a remainder term depending only on $F_\rho$ and $H_\sigma$ with $\rho$, $\sigma<\nu$. This suggests to consider for each $\nu\ge 2$ splittings of the form
$$
\ca H^\nu=\Im L_\Lambda|_{\ca H^\nu}\oplus\ca N^\nu\quad\hbox{and}\quad
\ca H^\nu=\Ker L_\Lambda|_{\ca H^\nu}\oplus\ca M^\nu
$$ 
where $\ca N^\nu$ and $\ca M^\nu$ are suitable complementary subspaces. Then, arguing by
induction (see Proposition~2.4), for each $\nu\ge 2$ it is possible to find a unique $H_\nu\in\ca M^\nu$
such that
$$
\{\Phi^{-1}\circ F\circ\Phi\}_\nu=F_\nu-L_\Lambda(H_\nu)+R_\nu\in\ca N^\nu\;;
\neweq\eqzuno
$$
we can then say that $G=\Phi^{-1}\circ F\circ\Phi$ is in {\sl first order normal form} with respect to the given
choice of complementary subspaces. 

When $\Lambda$ is diagonal, $\Ker L_\Lambda$ is
generated by the resonant monomials, and $\Im L_\Lambda$ is generated by the
non-resonant monomials; in particular, for each $\nu\ge 2$ we have the splitting
$$
\ca H^\nu=\Im L_\Lambda|_{\ca H^\nu}\oplus\Ker L_\Lambda|_{\ca H^\nu}\;.
$$
Thus taking $\ca N^\mu=\Ker L_\Lambda|_{\ca H^\nu}$ and $\ca M^\mu=\Im L_\Lambda|_{\ca H^\nu}$ we see that the classical Poincar\'e-Dulac normal form coincides with the first order normal 
form with respect to these complementary subspaces (when $\Lambda$ has a nilpotent
part the situation is only slightly more complicated; see Section~2 for details).

A consequence of \eqzuno\ is that if $H_\nu\in\Ker L_\Lambda$ then $\{\Phi^{-1}\circ F
\circ\Phi\}_\nu$ does not depend on~$H_\nu$; however, $H_\nu$ does affect the remainder
terms $R_\rho$ with $\rho>\nu$. In other words, we can use the terms $H_\sigma\in\Ker
L_\Lambda$ with $\sigma<\nu$ to simplify the remainder term $R_\nu$.

More precisely, if we take 
$F$ is in first order normal form, that is 
$$
F=\Lambda+\sum_{\nu\ge\mu} F_\nu
$$
with $F_\nu\in\ca N^\nu$ for all $\nu\ge \mu$ (and $F_\mu\ne O$), and take $\Phi\in\widehat\ca O^n_I$ such that $H_\nu\in\Ker L_\Lambda$ for all $\nu\ge 2$, it turns out that there is
an operator $L_{F_\mu,\Lambda}\colon\widehat\ca O^n\to\widehat\ca O^n$ sending each
$\ca H^{\nu-\mu+1}$ in $\ca H^\nu$ such that
$$
\{\Phi^{-1}\circ F\circ\Phi\}_\nu=F_\nu-L_{F_\mu,\Lambda}(H_{\nu-\mu+1})+R'_\nu
$$  
for all $\nu\ge\mu$, where $R'_\nu$ is a remainder term depending only on $F_\rho$ with $\rho<\nu$ and on $H_\sigma$ with $\sigma<\nu-\mu+1$  (see Theorem~2.3 for a more complete
formula valid without assumptions on $F$ and~$\Phi$). The operator $L_{F_\mu,\Lambda}$
is given by
$$
L_{F_\mu,\Lambda}(H)=\bigl((\Jac H)\circ\Lambda\bigr)\cdot F_\mu-(\Jac F_\mu)\cdot H\;;
$$
notice that, contrarily to $L_\Lambda$, the operator $L_{F_\mu,\Lambda}$ is different from
the operators appearing in the renormalization or hypernormalization of singular vector fields,
and thus it has to be studied on its own.

If the subspaces $\ca N^\nu$ are chosen (as will be in our case when $\Lambda$ is diagonalizable) so that 
$$
L_{F_\mu,\Lambda}
(\Ker L_\Lambda\cap\ca H^{\nu-\mu+1})\subseteq\ca N^\nu
\neweq\eqdd
$$ 
for all $\nu\ge\mu$
(notice that this condition is particularly easy to state if $\ca N^\nu=\Ker L_\Lambda\cap\ca H^\nu$), then $R'_\nu
\in\ca N^\mu$
for all $\nu\ge\mu$. Therefore we can argue as before: putting, for simplicity, $\ca H^\nu_\Lambda=
\Ker L_\Lambda\cap\ca H^\nu$, if we choose
splittings
$$
\ca N^\nu=\Im L_{F_\mu,\Lambda}|_{\ca H^{\nu-\mu+1}_\Lambda}\oplus\tilde\ca N^\nu
$$
and
$$
\ca H^{\nu-\mu+1}_\Lambda=\Ker L_{F_\mu,\Lambda}|_{\ca H^{\nu-\mu+1}_\Lambda}\oplus\tilde\ca M^{\nu-\mu+1}
$$
then arguing again by induction for each $\nu\ge\mu$ it is possible to find a unique $H_{\nu-\mu+1}\in\tilde\ca M^{\nu-\mu+1}$ such that
$$
\{\Phi^{-1}\circ F\circ\Phi\}_\nu=F_\nu-L_{F_\mu,\Lambda}(H_{\nu-\mu+1})+R'_\nu\in\tilde\ca N^\nu\;.
$$  
We shall then say that $G=\Phi^{-1}\circ F\circ\Phi$ is in {\sl renormalized} (or {\sl second order\/})
{\sl Poincar\'e-Dulac normal form,} with respect to the chosen complementary subspaces.

We are left with saying how to choose the complementary subspaces. In this paper, we shall use
the orthogonal subspaces with respect to the Fischer Hermitian product, defined by
$$
\langle z_1^{p_1}\cdots z_n^{p_n}e_h,z_1^{q_1}\cdots z_n^{q_n}e_k\rangle=
\cases{
0&if $h\ne k$ or $p_j\ne q_j$ for some $j$;\cr
\noalign{\smallskip}
\displaystyle {p_1!\cdots p_n!\over(p_1+\cdots+p_n)!}&if $h=k$ and $p_j=q_j$ for all $j$.\cr}
\neweq\eqzFi
$$
The reason of this choice is that, as we shall see in Sections~3 and~4, it will substantially simplify 
the expression of the renormalized Poincar\'e-Dulac normal forms. In particular, when $\Lambda=O$ and $n=2$, it turns out that, except in a few degenerate cases,  the renormalized Poincar\'e-Dulac normal forms depend on two power series of {\it one} variable only. 

\smallsect 1. Homogeneous maps

In this section we shall collect a few results on homogeneous polynomials and maps we shall need later. 

%%\Nota Da fare: estendere a gerarchie di operatori come per i tre giapponesi.
%
%\newthm Lemma \uuno: Let $L\colon V\to W$ be a linear map between two finite-dimensional
%complex vector spaces endowed with positive definite Hermitian products, and let
%$L^*\colon W\to V$ be the adjoint map. Then
%\smallskip
%\itm{(i)} $V=\Ker L\bigoperp\Im L^*$ and $W=\Ker L^*\bigoperp\Im L$;
%%\itm{(ii)} $\Ker L^*=\Ker(LL^*)$;
%%\item{\rm (iii)} if $\Sigma$ denotes the spectrum of $LL^*$ and $E_{LL^*}(\lambda)\subseteq W$ denotes
%%the eigenspace of $LL^*$ relative to $\lambda\in\C$, then $\Sigma\subset\R^+$ and
%%$\Im L=\bigoperp\limits_{\lambda\in\Sigma^*}E_{LL^*}(\lambda)$, where $\Sigma^*=\Sigma\setminus\{0\}$;
%\item{\rm (ii)} for every $w\in W$ there exist a unique $w_0\in\Ker L^*$ and a unique $v_0\in(\Ker L)^\perp$ such that $w=w_0+L(v_0)$. 
%%Furthermore, $\|w_0\|$, $\|w-w_0\|\le\|w\|$ and
%%$$
%%\|v_0\|\le{1\over\min\limits_{\lambda\in\Sigma^*}\sqrt{\lambda}}\|w-w_0\|\;.
%%$$
%
%\pf (i) If $v\in\Ker L$ and $w\in W$ we have
%$$
%\langle v,L^*(w)\rangle=\langle L(v),w\rangle=0\;,
%$$
%and so $\Ker L\subseteq(\Im L^*)^\perp$. Conversely, if $v\in(\Im L^*)^\perp$ we have
%$$
%0=\langle v,L^*(w)\rangle=\langle L(v),w\rangle
%$$
%for all $w\in W$, and hence $(\Im L^*)^\perp\subseteq\Ker L$. 
%
%Since $(L^*)^*=L$, we also have $\Ker L^*=(\Im L)^\perp$.
%
%%(ii) Clearly $\Ker L^*\subseteq\Ker(LL^*)$. Conversely, if $w\in\Ker(LL^*)$ we have
%%$$
%%0=\langle w,LL^*(w)\rangle=\langle L^*(w),L^*(w)\rangle=\|L^*(w)\|^2\;,
%%$$
%%and hence $w\in\Ker L^*$.
%%
%%(iii) The operator $LL^*$ is self-adjoint and positive semidefinite; hence $\Sigma\subset\R^+$ and
%%$W$ is the orthogonal sum of the eigenspaces of $LL^*$. In particular
%%$$
%%\bigoperp_{\lambda\in\Sigma^*}E_{LL^*}(\lambda)=\Ker(LL^*)^\perp=(\Ker L^*)^\perp=\Im L\;.
%%$$
%
%(ii) Given $w\in W$, by (i) 
%%and (iii) 
%we can decompose $w$ in a unique way as $w=w_0+w_1$, with $w_0\in\Ker L^*$ and $w_1\in
%\Im L$. 
%%$$
%%w=w_0+\sum_{\lambda\in\Sigma^*}w_\lambda
%%\neweq\equuno
%%$$ 
%%with $w_\lambda\in E_{LL^*}(\lambda)$. 
%Furthermore, (i) implies that $\Im L=L(\Im L^*)$ and that $L|_{\Im L^*}$ is injective; so there exists a unique $v_0\in\Im L^*=(\Ker L)^\perp$ such that
%$L(v_0)=w_1$.\qedn
%
%Since \equuno\ is an orthogonal decomposition, we have
%$$
%\|w\|^2=\|w_0\|^2+\|w-w_0\|^2=\|w_0\|^2+\sum_{\lambda\in\Sigma^*}\|w_\lambda\|^2;
%$$
%in particular $\|w\|\ge \|w_0\|$, $\|w-w_0\|$. Furthermore, if we set $v_\lambda=\lambda^{-1}
%L^*(w_\lambda)\in\Im L^*$ we get
%$$
%w=w_0+\sum_{\lambda\in\Sigma^*}w_\lambda=w_0+\sum_{\lambda\in\Sigma^*}{1\over\lambda}
%LL^*(w_\lambda)=w_0+L\left(\sum_{\lambda\in\Sigma^*}v_\lambda\right)\;;
%$$
%hence $v_0=\sum\limits_{\lambda\in\Sigma^*}v_\lambda$. Now,
%$$
%\langle v_\lambda,v_\mu\rangle={1\over\lambda\mu}\langle L^*(w_\lambda),L^*(w_\mu)\rangle
%={1\over\lambda\mu}\langle w_\lambda,LL^*(w_\mu)\rangle={1\over\lambda}\langle w_\lambda,
%w_\mu\rangle=\cases{0&if $\lambda\ne\mu$,\cr {1\over\lambda}\|w_\lambda\|^2&if $\lambda=\mu$;
%\cr}
%$$
%in particular, $v_\lambda\perp v_\mu$ if $\lambda\ne\mu$, and $\|v_\lambda\|={1\over\sqrt{\lambda}}\|w_\lambda\|$. Therefore
%$$
%\|v_0\|^2=\sum_{\lambda\in\Sigma^*}\|v_\lambda\|^2=\sum_{\lambda\in\Sigma^*}{1\over\lambda}
%\|w_\lambda\|^2\le{1\over\min\limits_{\lambda\in\Sigma^*}\lambda}\sum_{\lambda\in\Sigma^*}
%\|w_\lambda\|^2={1\over\min\limits_{\lambda\in\Sigma^*}\lambda}\|w-w_0\|^2\;,
%$$
%and we are done. \qedn

\newdef We shall denote by  $\ca H^d=\bigl(\C_d[z]\bigr)^n$ the 
space of {\sl homogenous maps of degree $d$,} i.e., of $n$-tuples of homogeneous polynomials of degree~$d\ge 1$ in the variables
$(z_1,\ldots,z_n)$. It is well known (see, e.g., [Car, pp. 79--88]) that to each $P\in\ca H^d$ is
associated a {\it unique} symmetric multilinear map $\tilde P\colon(\C^n)^d\to\C^n$ such that
$$
P(z)=\tilde P(z,\ldots,z)
$$
for all $z\in\C^n$. Notice that $\widehat\ca O^n=\prod\limits_{d\ge 1}\ca H^d$; we set $\ca H=\prod\limits_{d\ge 2}\ca H^d$.

%In particular, if $P\in\ca H^d$ and $Q\in\ca H^e$ then $Q\circ P\in\ca H^{de}$ and
%$$
%\widetilde{Q\circ P}(z_{11},\ldots,z_{d,e})=\tilde Q\bigl(\tilde P(z_{11},\ldots,z_{d,1}),\ldots,
%\tilde P(z_{1,e},\ldots,z_{d,e})\bigr)\;.
%$$

Roughly speaking, the symmetric multilinear map associated to a homogeneous map~$H$ encodes the derivatives of~$H$. For instance, we have 

\newthm Lemma \udue: If $H\in\ca H^d$ we have
$$
(\Jac H)(z)\cdot v=d\,\tilde H(v,z,\ldots,z)
$$ 
for all $z$, $v\in\C^n$.

\pf For $j=1,\ldots, n$ and $z\in\C^n$ we have
$$
{H(z+h e_j)-H(z)\over h}={\tilde H(z+he_j,\ldots,z+h e_j)-\tilde H(z,\ldots,z)\over h}
=d\,\tilde H(e_j,z,\ldots,z)+O(h)\;,
$$
where $e_j$ is the $j$-th vector of the canonical basis of $\C^n$. Therefore ${\de H\over\de z_j}(z)
=d\,\tilde H(e_j,z,\ldots,z)$ and
$$
(\Jac H)(z)\cdot v=\sum_{j=1}^n {\de H\over\de z_j}(z)v_j=d\sum_{j=1}^n\tilde H(e_j,z,\ldots,z)v_j
= d\,\tilde H(v,z,\ldots,z)\;.
$$
\qedn

Later on we shall need to compute the multilinear map associated to a homogeneous map
obtained as a composition. The formula we are interested in is contained in the next lemma.

\newthm Lemma \udueb: Assume that $P\in\ca H^d$ is of the form
$$
P(z)=\tilde K\bigl(H_{d_1}(z),\ldots,H_{d_r}(z)\bigr)\;,
$$
where $\tilde K$ is $r$-multilinear, $d_1+\cdots+d_r=d$, and $H_{d_j}\in\ca H^{d_j}$ for
$j=1,\ldots, r$. Then
$$
\tilde P(v,w,\ldots,w)={1\over d}\sum_{j=1}^r d_j\tilde K\bigl(H_{d_1}(w),\ldots,\tilde H_{d_j}(v,w,\ldots,w),
\ldots,H_{d_r}(w)\bigr)
$$
for all $v$, $w\in\C^n$.

\pf Write $z=w+\eps v$. Then
$$
\eqalign{P(w)&+d\eps\tilde P(v,w,\ldots,w)+O(\eps^2)\cr
&=P(w+\eps v)=
\tilde K\bigl(\tilde H_{d_1}(w+\eps v,\ldots,w+\eps v),\ldots,\tilde H_{d_r}(w+\eps v,\ldots,
w+\eps v)\bigr)\cr
&=\tilde K\bigl(H_{d_1}(w),\ldots,H_{d_r}(w)\bigr)\!+\eps\sum_{j=1}^r \!d_j
\tilde K\bigl(H_{d_1}(w),\ldots,\tilde H_{d_j}(v,w,\ldots,w),\ldots,H_{d_r}(w)\bigr)+O(\eps^2)\;,
\cr}
$$
and we are done.\qedn

\newdef Given a linear map $\Lambda\in M_{n,n}(\C)$, we define a linear operator 
$L_\Lambda\colon\ca H\to\ca H$ by setting
$$
L_\Lambda(H)=H\circ\Lambda -\Lambda H\;.
$$
We shall say that a homogeneous map $H\in\ca H^d$ is {\sl $\Lambda$-resonant} if $L_\Lambda(H)=O$, and we shall denote by $\ca H^d_\Lambda=\Ker L_\Lambda\cap \ca H^d$ the 
subspace of $\Lambda$-resonant homogeneous maps of degree~$d$. Finally,
we set $\ca H_\Lambda=\prod\limits_{d\ge 2}\ca H^d_\Lambda$. 

When $\Lambda$ is diagonal, then the $\Lambda$-resonant monomials are exactly the
resonant monomials appearing in the classical Poincar\'e-Dulac theory.

\newdef If $Q=(q_1,\ldots,q_n)\in\N^n$ is a multi-index
and $z=(z_1,\ldots,z_n)\in\C^n$, we shall put $z^Q=z_1^{q_1}\cdots z_n^{q_n}$. Given
$\Lambda=\diag(\lambda_1,\ldots,\lambda_n)\in M_{n,n}(\C)$, we shall say that $Q\in\N^n$ with $q_1+\cdots+q_n\ge 2$
is {\sl $\Lambda$-resonant} on the $j$-th coordinate if $\lambda_1^{q_1}\cdots
\lambda_n^{q_n}=\lambda_j$. We shall
denote by $\Res_j(\Lambda)$ the set of multi-indices $\Lambda$-resonant on the $j$-th coordinate.

\newrem If $\Lambda=\diag(\lambda_1,\ldots,\lambda_n)\in M_{n,n}(\C)$ is diagonal, and $z^Qe_j
\in\ca H^d$ is a homogeneous monomial (with $q_1+\cdots+q_n=d$), then (identifying the matrix $\Lambda$ with the vector, still denoted by $\Lambda$, of its diagonal entries) we have 
%$H_{Q,j}\circ\Lambda(z)=\Lambda^Q H_{Q,j}(z)$ and $\Lambda H_{Q,j}(z)=\lambda_j H_{Q,j}(z)$. 
%In particular,
$$
L_\Lambda(z^Qe_j)=(\Lambda^Q-\lambda_j)z^Qe_j\;.
$$
Therefore $z^Qe_j$ is $\Lambda$-resonant if and only if $Q$ is $\Lambda$-resonant in the $j$-th coordinate, that is if and only if
$Q\in\Res_j(\Lambda)$. In particular, a basis of $\ca H^d_\Lambda$ is given by $z^Qe_j$ with
$Q\in\Res_j(\Lambda)$ and $q_1+\cdots+q_n=d$, and we have
$$
\ca H^d=\ca H^d_\Lambda\oplus\Im L_\Lambda|_{\ca H^d}
$$
for all $d\ge 2$.

It is possible to detect the $\Lambda$-resonance by using the associated multilinear map:

\newthm Lemma \utre: If $\Lambda\in M_{n,n}(\C)$ and $H\in\ca H^d$ then $H$ is
$\Lambda$-resonant if and only if
$$
\tilde H(\Lambda v_1,\ldots,\Lambda v_d)=\Lambda\tilde H(v_1,\ldots,v_d)
\neweq\equdue
$$
for all $v_1,\ldots,v_d\in\C^n$. In particular, if $H\in\ca H^d_\Lambda$ then
$$
\bigl((\Jac H)\circ\Lambda\bigr)\cdot\Lambda=\Lambda\cdot(\Jac H)\;.
\neweq\equtre
$$

\pf One direction is trivial. Conversely, assume $H\in\ca H^d_\Lambda$. By definition, $H$ is $\Lambda$-resonant if and only if $\tilde H(\Lambda w,\ldots,\Lambda w)
=\Lambda\tilde H(w,\ldots,w)$ for all $w\in\C^n$. Put $w=z+\eps v_1$; then
$$
\eqalign{\tilde H(\Lambda z,\ldots,\Lambda z)+\eps d\,\tilde H(\Lambda v_1,\Lambda z,\ldots,
\Lambda z)+O(\eps^2)&=\tilde H\bigl(\Lambda(z+\eps v_1),\ldots,\Lambda(z+\eps v_1)\bigr)\cr
&=\Lambda\tilde H(z+\eps v_1,\ldots,z+\eps v_1)\cr
&=\Lambda\tilde H(z,\ldots,z)+\eps d\,\Lambda\tilde H(v_1,z,\ldots,z)+O(\eps^2)\;,\cr}
$$
and thus
$$
\tilde H(\Lambda v_1,\Lambda z,\ldots,\Lambda z)=\Lambda\tilde H(v_1,z,\ldots,z)\;;
\neweq\equdueb
$$
in particular \equtre\ is a consequence of Lemma~\udue.

Now put $z=z_1+\eps v_2$ in \equdueb. We get
$$
\eqalign{\tilde H(\Lambda v_1,\Lambda z_1,\ldots,\Lambda z_1)&+\eps (d-1)\tilde H(\Lambda v_1,\Lambda v_2,\Lambda z_1,\ldots,
\Lambda z_1)+O(\eps^2)\cr
&=\tilde H\bigl(\Lambda v_1,\Lambda(z_1+\eps v_2),\ldots,\Lambda(z_1+\eps v_2)\bigr)\cr
&=\Lambda\tilde H(v_1,z_1+\eps v_2,\ldots,z_1+\eps v_2)\cr
&=\Lambda\tilde H(v_1,z_1,\ldots,z_1)+\eps (d-1)\Lambda\tilde H(v_1,v_2,z,\ldots,z)+O(\eps^2)\;,\cr}
$$
and hence
$$
\tilde H(\Lambda v_1,\Lambda v_2,\Lambda z_1,\ldots,\Lambda z_1)=\Lambda\tilde H(v_1,v_2,z_1,\ldots,z_1)
$$
for all $v_1$, $v_2$, $z_1\in\C^n$. Proceeding in this way we get \equdue.
\qedn

As we shall see in the next section, the operator $L_\Lambda$ appears in the usual
Poincar\'e-Dulac normalization; for the renormalization we shall need a different
operator, that we now introduce.

\newdef Given $P\in\ca H^\mu$ and $\Lambda\in M_{n,n}(\C)$, let $L_{P,\Lambda}\colon
\ca H^d\to\ca H^{d+\mu-1}$ be given by
$$
L_{P,\Lambda}(H)(z)=d\,\tilde H\bigl(P(z),\Lambda z,\ldots,
\Lambda z\bigr)-\mu\tilde P\bigl(H(z),z,\ldots,z\bigr)\;.
$$

\newrem Lemma \udue\ implies that
$$
d\,\tilde H\bigl(P(z),\Lambda z,\ldots,\Lambda z\bigr)=(\Jac H)(\Lambda z)\cdot P(z)\;.
$$
Therefore
$$
L_{P,\Lambda}(H)=\bigl((\Jac H)\circ\Lambda\bigr)\cdot P-(\Jac P)\cdot H\;.
$$
In particular, when $\Lambda=O$ we have 
$$
L_{P,O}(H)=-(\Jac P)\cdot H\;.
$$

\newrem If we take $\mu=1$ and $P=\Lambda$ we find
$$
L_{\Lambda,\Lambda}(H)=d\tilde H(\Lambda,\ldots,\Lambda)-\Lambda H
=(d-1)H\circ\Lambda+L_\Lambda(H)\;;
$$
in particular, $L_{\Lambda,\Lambda}\ne L_\Lambda$.

As mentioned in the introduction, for our machinery to work is important that the operator
$L_{P,\Lambda}$ sends the kernel of $L_\Lambda$ into itself. This is the last result
of this section:

\newthm Corollary \uqua: Take $\Lambda\in M_{n,n}(\C)$ and $P\in\ca H^\mu_\Lambda$.
Then $L_{P,\Lambda}(\ca H^d_\Lambda)\subseteq\ca H^{d+\mu-1}_\Lambda$ for all $d\ge 2$.

\pf Using Lemma~\utre\ and the definition of $L_{P,\Lambda}$, if $H\in\ca H^d_\Lambda$ we get
$$
\eqalign{
L_{P,\Lambda}(H)(\Lambda z)&=d\,\tilde H\bigl(P(\Lambda z),\Lambda^2 z,\ldots,\Lambda^2 z\bigr)
-\mu\tilde P\bigl(H(\Lambda z),\Lambda z,\ldots,\Lambda z\bigr)\cr
&=d\,\tilde H\bigl(\Lambda P(z),\Lambda^2 z,\ldots,\Lambda^2 z\bigr)
-\mu\tilde P\bigl(\Lambda H(z),\Lambda z,\ldots,\Lambda z\bigr)\cr
&=d\,\Lambda\tilde H\bigl(P(z),\Lambda z,\ldots,\Lambda z\bigr)
-\mu\Lambda \tilde P\bigl(H(z),z,\ldots,z\bigr)\cr
&=\Lambda L_{P,\Lambda}(H)(z)\;.
\cr}
$$ 
\qedn

\smallsect 2. Renormalization

The aim of this section is to describe a procedure associating a renormalized formal Poincar\'e-Dulac
normal form to any germ of holomorphic (or even formal) self-map of $\C^n$ fixing the origin.
This is particularly interesting in the case of germs superattracting (i.e., with vanishing linear part) or tangent to the identity (i.e., with identity linear part), because in those cases all
monomials are resonant and so the usual
Poincar\'e-Dulac procedure just gives back the original germ.

The idea is the following. Studying the
classical proof (see, e.g., [Ar], [R1, 2] and Proposition~2.4 below) of the standard Poincar\'e-Dulac normalization of a 
germ $F$, 
it is clear that we find a unique formal germ $\Psi$ tangent to the identity and containing only
{\it nonresonant} monomials such that $F_1=\Psi^{-1}\circ F\circ\Psi$ is in Poincar\'e-Dulac normal
form, that is contains only resonant monomials. Choosing suitable positive
definite Hermitian products on the spaces of homogeneous polynomial maps, we shall then
be able to determine a {\it unique} formal germ $\Phi$ tangent to the identity and containing
only {\it resonant} monomials such that $\Phi^{-1}\circ F_1\circ\Phi$ is (in a precise sense)
a renormalized Poincar\'e-Dulac normal form of $F$.

Let us fix a few definitions and notations. 

\newdef We shall denote by $\widehat\ca O^n$
the space of $n$-tuples 
of formal power series with vanishing constant term. Furthermore, given $\Lambda\in M_{n,n}(\C)$ we shall denote by $\widehat\ca O^n_\Lambda$ the subset of~$F\in\widehat\ca O^n$ with $dF_O=\Lambda$.

\newdef Every $F\in\widehat\ca O^n$ can be written in a unique way
as a formal sum
$$
F=\sum_{d\ge 1} F_d
\neweq\eqduno
$$
with $F_d\in\ca H^d$; \eqduno\ is the {\sl homogeneous expansion} of $F$, and $F_d$ 
is the {\sl $d$-homogeneous term} of $F$. We shall often write $\{F\}_d$ for $F_d$. In particular,
if $F\in\widehat\ca O^n_\Lambda$ then $\{F\}_1=\Lambda$.

The homogeneous terms behave in a predictable way with respect to composition and inverse:

\newthm Lemma \duno: Take $F$, $G\in\widehat\ca O^n_O$, and let $F=\sum\limits_{d\ge 1} F_d$ and
$G=\sum\limits_{d\ge 1} G_d$ be their homogeneous expansions. Then
$$
\{F\circ G\}_d=\sum_{{1\le r\le d}\atop{d_1+\cdots+d_r=d}}\tilde F_r(G_{d_1},\ldots, G_{d_r})
$$
for all $d\ge 1$.

\pf See, e.g., [LS, Lemma A.4]. \qedn

\newthm Lemma \ddue: Take $\Phi\in\widehat\ca O^n_I$ with homogeneous expansion
$\Phi=I+\sum\limits_{d\ge\delta}H_d$, for some $\delta\ge 2$, and let $\Phi^{-1}=I+\sum\limits_{d\ge 2}K_d$
be the homogeneous expansion of the inverse. Then 
$$
K_d=
-H_d-\sum_{{2\le r\le d-1}\atop{d_1+\cdots+d_r=d}}\tilde K_r(H_{d_1},\ldots,H_{d_r})
\neweq\eqddue
$$
for all $d\ge 2$. In particular, $K_\delta=-H_\delta$, and $K_d=O$ for $d=2,\ldots,\delta-1$.
Furthermore, if $H_2,\ldots, H_d$ are $\Lambda$-resonant for some $\Lambda\in M_{n,n}(\C)$
then also $K_d$ is. 

\pf Lemma~\duno\ yields
$$
\sum_{{1\le r\le d}\atop{d_1+\cdots+d_r=d}}\tilde K_r(H_{d_1},\ldots,H_{d_r})=\{\Phi^{-1}\circ
\Phi\}_d=O
\neweq\eqdtre
$$
for all $d\ge 2$. Now, when $r=1$ we necessarily have $d_1=d$, and so $\tilde K_1(H_d)=H_d$
because $K_1=I$. Analogously, when $r=d$ we necessarily have $d_1=\cdots=d_r=1$, and so
$\tilde K_d(H_1,\ldots,H_1)=K_d$ because $H_1=I$. Therefore \eqdtre\ becomes
$$
H_d+\sum_{{2\le r\le d-1}\atop{d_1+\cdots+d_r=d}}\tilde K_r(H_{d_1},\ldots,H_{d_r})+K_d=O\;,
$$
and \eqddue\ follows. In particular, if $2\le d\le\delta$ in the sum in \eqddue\ we have $2\le d_j<\delta$
(and hence $H_{d_j}=O$) for at least one $j=1,\ldots,r$; thus $K_d=-H_d$ for $2\le d\le\delta$,
as claimed.

Finally, to prove the last assertion we argue by induction. Assume that $H_2,\ldots, H_d$ are
$\Lambda$-resonant. If $d=\delta$ then $K_\delta=-H_\delta$ and
thus $K_\delta$ is clearly $\Lambda$-resonant. Assume the assertion true for $d-1$; in particular,
$K_\delta,\ldots,K_{d-1}$ are $\Lambda$-resonant. Then
$$
\eqalign{K_d\circ\Lambda&=-H_d\circ\Lambda-\sum_{{2\le r\le d-1}\atop{d_1+\cdots+d_r=d}}\tilde K_r(H_{d_1}\circ\Lambda,\ldots,H_{d_r}\circ\Lambda)\cr
&=\Lambda H_d-\sum_{{2\le r\le d-1}\atop{d_1+\cdots+d_r=d}}\tilde K_r(\Lambda H_{d_1},\ldots,\Lambda H_{d_r})=\Lambda K_d\cr}
$$
because $K_2,\ldots,K_{d-1}$ are $\Lambda$-resonant (and we are using Lemma~\utre).
\qedn

\newdef Given $\Lambda\in M_{n,n}(\C)$, we shall say that $F\in\widehat\ca O^n$ is 
{\sl $\Lambda$-resonant} if $F\circ\Lambda=\Lambda F$. Clearly, $F$ is $\Lambda$-resonant
if and only if $\{F\}_d\in\ca H^d_\Lambda$ for all $d\in\N$. 

%We shall need the following technical lemma: 
%
%\newthm Lemma \dtre: Given $\Lambda\in M_{n,n}(\C)$, let $\Phi\in\widehat\ca O^n_I$ be
%$\Lambda$-resonant, and let $\Phi=I+\sum\limits_{d\ge 2}H_d$ and $\Phi^{-1}=I+
%\sum\limits_{d\ge 2}K_d$ be
%the homogeneous expansions of $\Phi$ and its inverse. Then
%$$
%\sum_{{2\le r\le d-1}\atop{d_1+\cdots+d_r=d}}\tilde K_r(\Lambda H_{d_1},\ldots,\Lambda H_{d_r})
%=O
%$$
%for all $d\ge 2$.
%
%\pf Since $\Phi$ is $\Lambda$-resonant we have $\Phi^{-1}\circ\Lambda\circ\Phi=\Lambda$, and hence $\{\Phi^{-1}\circ\Lambda\circ\Phi\}_d=O$ for all $d\ge 2$. But $\{\Lambda\circ\Phi\}_d=
%\Lambda H_d$ for all $d\ge 1$; therefore
%$$
%\{\Phi^{-1}\circ\Lambda\circ\Phi\}_d=\sum_{{1\le r\le d}\atop{d_1+\cdots+d_r=d}}\tilde K_r(\Lambda H_{d_1},\ldots,\Lambda H_{d_r})=O\;.
%$$
%To conclude, just notice that the summand for $r=1$ is $\Lambda H_d$,
%and the summand for $r=d$ is $\tilde K_d(\Lambda,\ldots,\Lambda and we are done.\qedn
%
%\Nota In realt\`a questo lemma non viene poi usato.

The main technical result of this section is the following:

\newthm Theorem \dquattro: Given $F\in\widehat\ca O^n_O$, let
$F=\Lambda+\sum\limits_{d\ge\mu}F_d$ be its homogeneous expansion, with $F_\mu\ne O$.
Then for every $\Phi\in\widehat\ca O^n_I$ with homogeneous
expansion $\Phi=I+\sum\limits_{d\ge 2}H_d$ and every $\nu\ge 2$ we have
$$
\{\Phi^{-1}\circ F\circ\Phi\}_\nu=F_\nu-L_\Lambda(H_\nu)-L_{F_\mu,\Lambda}(H_{\nu-\mu+1})+Q_\nu+R_\nu\;,
\neweq\eqdqua
$$
where $Q_\nu$ depends only on $\Lambda$ and on $H_\gamma$ with $\gamma<\nu$, while $R_\nu$ depends only on $F_\rho$ with $\rho<\nu$ and on $H_\gamma$ with $\gamma<\nu-\mu+1$, and we put $L_{F_\mu,\Lambda}(H_1)=O$. Furthermore,
we have:
\smallskip
\itm{(i)} if $H_2,\ldots,H_{\nu-1}\in\ca H_\Lambda$ then $Q_\nu=O$; in particular, if $\Phi$ is $\Lambda$-resonant then $L_\Lambda(H_\nu)=Q_\nu=O$
for all $\nu\ge 2$;
\itm{(ii)} if $\Phi$ is $\Lambda$-resonant then $\{\Phi^{-1}\circ F\circ\Phi\}_\nu=O$ for $2\le \nu<\mu$, $\{\Phi^{-1}\circ F\circ\Phi\}_\mu=
F_\mu$, and 
$$
\{\Phi^{-1}\circ F\circ\Phi\}_{\mu+1}=F_{\mu+1}-L_{F_\mu,\Lambda}(H_2)\;;
$$
\itm{(iii)} if $F=\Lambda$ then $R_\nu=O$ for all $\nu\ge 2$;
\item{\rm(iv)} if $F_2,\ldots, F_{\nu-1}$ and $H_2,\ldots,H_{\nu-\mu}$ are $\Lambda$-resonant
then $R_\nu$ is $\Lambda$-resonant.

\pf Using twice Lemma~\duno\ we get
$$
\eqalign{\{\Phi^{-1}\circ F\circ\Phi\}_\nu&=\!\!\!\!\!\!\!
\sum_{{1\le s\le\nu}\atop{\nu_1+\cdots+\nu_s=\nu}}\!\!\!
\tilde K_s(\{F\circ\Phi\}_{\nu_1},\ldots,\{F\circ\Phi\}_{\nu_s})\cr
&=\!\!\!\!\!\!\!\sum_{{1\le s\le\nu}\atop{\nu_1+\cdots+\nu_s=\nu}}
\!\sum_{{1\le r_1\le\nu_1}\atop{d_{11}+\cdots+d_{1r_1}=\nu_1}}\!\!\!\!\!\cdots\!\!\!\!
\sum_{{1\le r_s\le\nu_s}\atop{d_{s1}+\cdots+d_{sr_s}=\nu_s}}\!\!\!\!\!\!\!\!\!\!\!\!\!
\tilde K_s\bigl(\tilde F_{r_1}(H_{d_{11}},\ldots,\!H_{d_{1r_1}}),\ldots,
\tilde F_{r_s}(H_{d_{s1}},\!\ldots,\!H_{d_{sr_s}})\bigr)\cr
&=T_\nu+S_1(\nu)+\sum_{s\ge 2} S_s(\nu)\;,
\cr}
$$
where $\Phi^{-1}=I+\sum\limits_{d\ge 2}K_d$ is the homogeneous expansion
of $\Phi^{-1}$, and:
$$
T_\nu=\sum_{{1\le s\le\nu}\atop{\nu_1+\cdots+\nu_s=\nu}}\!\!\!\tilde K_s(
\Lambda H_{\nu_1},\ldots,\Lambda H_{\nu_s})
\leqno(1)
$$
is obtained considering only the terms with $r_1=\ldots=r_s=1$; 
$$
S_1(\nu)=\sum_{{\mu\le r\le\nu}\atop{d_1+\cdots+d_r=\nu}}\!\!\!
\tilde F_r(H_{d_1},\ldots, H_{d_r})
\leqno (2)
$$
contains the terms with $s=1$ and $r_1>1$; and
$$
S_s(\nu)=\sum_{\nu_1+\cdots+\nu_s=\nu}\!\!
\sum_{{{{1\le r_1\le\nu_1}\atop{\vdots}}\atop{1\le r_s\le\nu_s}}\atop
{\max\{r_1,\ldots,r_s\}\ge\mu}}
\sum_{{{d_{11}+\cdots+d_{1r_1}=\nu_1}\atop{\vdots}}\atop{d_{s1}+\cdots
+d_{sr_s}=\nu_s}}\!\!\!\tilde K_s\bigl(\tilde F_{r_1}(H_{d_{11}},\ldots,
H_{d_{1r_1}}),\ldots,\tilde F_{r_s}(H_{d_{s1}},\ldots,H_{d_{sr_s}})\bigr)
\leqno(3)
$$
contains the terms with fixed $s\ge 2$ and at least one $r_j$ greater than 1
(and thus greater than or equal to $\mu$, because $F_2=\ldots=F_{\mu-1}=O$
by assumption). 

Let us first study $T_\nu$. The summand corresponding to $s=1$ is
$\Lambda H_\nu$; the summand corresponding to $s=\nu$ is $K_\nu\circ\Lambda$; therefore
$$
T_\nu=\Lambda H_\nu+K_\nu\circ\Lambda+\sum_{{2\le s\le\nu-1}\atop{\nu_1+\cdots+\nu_s=\nu}}\!\!\!\tilde K_s(
\Lambda H_{\nu_1},\ldots,\Lambda H_{\nu_s})=-L_\Lambda(H_\nu)+Q_\nu\;,
$$ 
where, using Lemma~\ddue\ to express $K_\nu$,
$$
Q_\nu=\sum_{{2\le s\le\nu-1}\atop{\nu_1+\cdots+\nu_s=\nu}}\!\!\!
\left[\tilde K_s(
\Lambda H_{\nu_1},\ldots,\Lambda H_{\nu_s})-
\tilde K_s(H_{\nu_1}\circ\Lambda,\ldots H_{\nu_s}\circ\Lambda)
\right]
$$
depends only on $\Lambda$ and $H_\gamma$ with $\gamma<\nu$ because $2\le s
\le\nu-1$ in the sum. In particular, if $H_1,\ldots,H_{\nu-1}\in\ca H_\Lambda$ then $Q_\nu=O$, and (i) is proved.

Now let us study $S_1(\nu)$. First of all, we clearly have $S_1(\nu)=O$
for $2\le\nu<\mu$, and $S_1(\mu)=F_\mu$. When $\nu>\mu$ we can write
$$
\eqalign{S_1(\nu)&=F_\nu+\sum_{{\mu\le r\le\nu-1}\atop{d_1+\cdots+d_r=\nu}}
\!\!\!\tilde F_r(H_{d_1},\ldots, H_{d_r})\cr
&=F_\nu+\mu\tilde F_\mu(H_{\nu-\mu+1},I,\ldots,I)+\!\!\!\!\!\!\!
\sum_{{d_1+\cdots+d_\mu=
\nu}\atop{1<\max\{d_j\}<\nu-\mu+1}}\!\!\!\!\!\!\tilde F_\mu(H_{d_1},\ldots, H_{d_\mu})
+\!\!\!\sum_{{\mu+1\le r\le\nu-1}\atop{d_1+\cdots+d_r=\nu}}
\!\!\!\tilde F_r(H_{d_1},\ldots, H_{d_r})\;.
\cr}
$$
in particular, $S_1(\mu+1)=F_{\mu+1}+\mu\tilde F_\mu(H_2,I,\ldots,I)$. Notice that the two remaining sums depend only on 
$F_\rho$ with $\rho<\nu$ and on $H_\gamma$ with $\gamma<\nu-\mu+1$
(in the first sum is clear; for the second one, if $d_j\ge\nu-\mu+1$
for some $j$ we then would have $d_1+\cdots+d_r\ge\nu-\mu+1+r-1\ge\nu+1$,  
impossible). Summing up we have
$$
S_1(\nu)=\cases{O&for $2\le\nu<\mu$,\cr
F_\mu&for $\nu=\mu$,\cr
F_{\mu+1}+\mu\tilde F_\mu(H_2,I,\ldots,I)&for $\nu=\mu+1$,\cr
F_\nu+\mu\tilde F_\mu(H_{\nu-\mu+1},I,\ldots,I)+R^1_\nu&for $\nu>\mu+1$,
\cr}
$$
where
$$
R^1_\nu=\!\!\!\sum_{{d_1+\cdots+d_\mu=
\nu}\atop{1<\max\{d_j\}<\nu-\mu+1}}\!\!\!\tilde F_\mu(H_{d_1},\ldots, H_{d_\mu})
+\sum_{{\mu+1\le r\le\nu-1}\atop{d_1+\cdots+d_r=\nu}}
\!\!\!\tilde F_r(H_{d_1},\ldots, H_{d_r})
$$
depends only on 
$F_\rho$ with $\rho<\nu$ and on $H_\gamma$ with $\gamma<\nu-\mu+1$. 

Let us now discuss $S_s(\nu)$ for $s\ge 2$. First of all, the condition
$\max\{r_1,\ldots,r_s\}\ge\mu$ implies
$$
\mu+s-1\le r_1+\cdots+r_s\le\nu_1+\cdots+\nu_s=\nu\;,
$$
that is $s\le\nu-\mu+1$. In particular, $S_s(\nu)=O$ if $\nu\le\mu$ or if
$s>\nu-\mu+1$. %, and
%$$
%\{\Phi^{-1}\circ F\circ\Phi\}_\nu=T_\nu+S_1(\nu)+\cdots+S_{\nu-\mu+1}(\nu).
%$$
Moreover, if we had $d_{ij}\ge\nu-\mu+1$ for some $1\le i\le
s$ and $1\le j\le r_s$ we would get
$$
\nu=d_{11}+\cdots+d_{sr_s}\ge\nu-\mu+1+r_1+\cdots+r_s-1
\ge\nu-\mu+1+\mu+s-1-1=\nu+s-1>\nu\;,
$$
impossible. This means that $S_s(\nu)$ depends only on $F_\rho$ with 
$\rho<\nu$ for all $s$, on $H_\gamma$ with $\gamma<\nu-\mu+1$ when $s<\nu-\mu+1$,
and that $S_{\nu-\mu+1}(\nu)$ depends on $H_{\nu-\mu+1}$ only because
it contains $\tilde K_{\nu-\mu+1}$. Furthermore, the
conditions $\max\{r_1,\ldots,r_{\nu-\mu+1}\}\ge\mu$ and $\nu_1+\ldots+\nu_{\nu-\mu+1}=\nu$ imply
that
$$
S_{\nu-\mu+1}(\nu)=(\nu-\mu+1)\tilde K_{\nu-\mu+1}(F_\mu,\Lambda,\ldots,
\Lambda)=-(\nu-\mu+1)\tilde H_{\nu-\mu+1}(F_\mu,\Lambda,\ldots,\Lambda)+R^2_\nu\;,
$$
where (using Lemmas~\udueb\ and~\ddue)
$$
R^2_\nu=\sum_{{2\le r\le\nu-\mu}\atop{d_1+\cdots+d_r=\nu-\mu+1}}
\sum_{j=1}^r d_j\tilde K_r\bigl(H_{d_1}\circ\Lambda,\ldots,\tilde H_{d_j}(F_\mu,\Lambda,\ldots,
\Lambda),\ldots,H_{d_r}\circ\Lambda\bigr)
$$ 
depends only on $\Lambda$, $F_\mu$ and $H_\gamma$ with
$\gamma<\nu-\mu+1$.

Putting everything together, we have
$$
\eqalign{
\{\Phi^{-1}\circ F\circ\Phi\}_\nu&=T_\nu+S_1(\nu)+\sum_{s=2}^{\nu-\mu+1}
S_s(\nu)\cr
&=F_\nu-L_\Lambda(H_\nu)+Q_\nu+\cases{O&if $2\le\nu\le\mu$,\cr
-L_{F_\mu,\Lambda}(H_2)&if $\nu=\mu+1$,\cr
-L_{F_\mu,\Lambda}(H_{\nu-\mu+1})+R_\nu&if $\nu>\mu+1$,\cr}
\cr}
$$
where
$$
R_\nu=R^1_\nu+R^2_\nu+\sum_{s=2}^{\nu-\mu}S_s(\nu)
$$
depends only on $F_\rho$ with $\rho<\mu$ and on $H_\gamma$ with $\gamma<
\nu-\mu+1$. In particular, if $F=\Lambda$ then we have $S_s(\nu)=O$ for all $s\ge 1$ and hence
$R_\nu=O$ for all $\nu\ge 2$. 

In this way we have proved \eqdqua\ and parts (i), (ii) and (iii). 
Concerning (iv), it suffices to notice that if $F_2,\ldots,F_{\nu-1}$ and $H_2,\ldots, H_{\nu-\mu+1}$
are $\Lambda$-resonant, then also $R^1_\nu$, $S_2(\nu),\ldots,S_{\nu-\mu}(\nu)$ and
$R^2_\nu$ (by Lemmas~\utre\ and~\ddue) are $\Lambda$-resonant.\qedn

We can now prove the existence of a first order normalization in the sense described in the
introduction.

\newthm Proposition \foPD: Take $\Lambda\in M_{n,n}(\C)$ and for each $\nu\ge2$ choose 
two subspaces $\ca N^\nu$,~$\ca M^\nu\subseteq\ca H^\nu$ such that 
$\ca H^\nu=\Im L_\Lambda|_{\ca H^\nu}\oplus\ca N^\nu$ and $\ca H^\nu=\ca H^\nu_\Lambda\oplus\ca M^\nu$. Then for every $F\in\widehat\ca O^n_\Lambda$ there exists a unique $\Phi=I+\sum\limits_{d\ge 2}H_d$ such that $H_d\in\ca M^d$ for all $d\ge 2$ and $\{\Phi^{-1}\circ F\circ\Phi\}_\nu\in\ca N^\nu$ for all $\nu\ge 2$.

\pf Notice that, by construction, $L_\Lambda(\ca H^\nu)=L_\Lambda(\ca M^\nu)$ and $L_\Lambda|_{\ca M^\nu}$ is injective. Now put $G=\Phi^{-1}\circ F\circ\Phi$; we define $H_d$ by induction. For $d=2$, we see that there exist a unique $G\in\ca N^2$ and a unique $H\in\ca M^2$ such that $F_2=G+L_\Lambda(H)$. Since \eqdqua\ says that
$$
G_2=F_2-L_\Lambda(\{\Phi\}_2)=G+L_\Lambda(H)-L_\Lambda(\{\Phi\}_2)\;,
$$
to get $G_2\in\ca N^2$ with $\{\Phi\}_2\in\ca M^2$ we must take
$\{\Phi\}_2=H$.

Assume now that we have defined $H_j\in\ca M^j$ for $j=2,\ldots,H_{d-1}$. In 
particular, this determines completely the terms $Q_d$, $R_d$ and $L_{F_2,\Lambda}(H_{d-1})$
in \eqdqua. So there exist a unique $G\in\ca N^d$ and a unique $H\in\ca M^d$ such that $F_d-L_{F_2,\Lambda}(H_{d-1})+Q_d+R_d=G+L_\Lambda(H)$. Then
to get $G_d\in\ca N^d$ with $\{\Phi\}_d\in\ca M^d$ the 
only choice is $\{\Phi\}_d=H$, and thus $G_d=G$.\qedn

There are a few natural choices for the subspaces $\ca N^\nu$ and $\ca M^\nu$ (see, e.g.,
[Mu1, Chapter~4]). If $\Lambda$ is diagonal, then Remark~1.1 shows that we can take
$\ca N^\nu=\ca H^\nu_\Lambda$ and $\ca M^\nu=\Im L_\Lambda|_{\ca H^\nu}$, and thus 
Proposition~\foPD\ gives nothing but the usual Poincar\'e-Dulac normal form.

Another possibility arises choosing on each $\ca H^\nu$ a positive definite Hermitian product. Then, denoting by $L^*_\Lambda$ the adjoint operator
of $L_\Lambda$, we have
$$
\ca H^\nu=\Im L_\Lambda|_{\ca H^\nu}\bigoperp\Ker L^*_\Lambda|_{\ca H^\nu}
=\ca H^\nu_\Lambda\bigoperp\Im L^*_\Lambda|_{\ca H^\nu}\;,
$$
and thus we can take $\ca N^\nu=\Ker L_\Lambda^*|_{\ca H^\nu}$ and $\ca M^\nu=\Im L^*_\Lambda|_{\ca H^\nu}$. 

If we use the Fischer Hermitian product introduced in \eqzFi, it turns out that $L^*_\Lambda=L_{\Lambda^*}$, where $\Lambda^*$ is the matrix adjoint of~$\Lambda$ (see, e.g., [Mu1, Lemma 4.6.6]). Furthermore, when $\Lambda$ is diagonal we clearly have $\Ker L_{\Lambda^*}=\Ker L_\Lambda$, and thus we have again recovered the usual Poincar\'e-Dulac normal form. More generally, if $\Lambda=D+N$ is in Jordan normal form, with $D$ diagonal and $N$ nilpotent, then $\Ker L^*_\Lambda=\Ker L_D\cap\Ker L_{N^*}\subseteq\Ker L_D$ (see, e.g.,
[Mu1, Lemma 4.6.9]), and
thus in this case too we have recovered the usual Poincar\'e-Dulac normal form (composed
by monomials resonant with respect to the eigenvalues of~$\Lambda$, i.e., $D$-resonant).

We can now introduce the renormalized Poincar\'e-Dulac normal form.

\newdef Given $\Lambda\in M_{n,n}(\C)$, we shall say that a $G\in\widehat\ca O^n_\Lambda$ is 
{\sl in renormalized Poincar\'e-Dulac normal form} if $G=\Lambda$ or the homogeneous expansion $G=\Lambda+\sum\limits_{d\ge\mu}G_d$ of $G$ satisfies the following 
conditions:
\smallskip
\item{(a)} $G_\mu\in\ca H^\mu_\Lambda\setminus\{O\}$;
\item{(b)} $G_d\in\ca H^d_\Lambda\cap(\Im L_{G_\mu,\Lambda})^\perp$ for all
$d>\mu$ (where we are using the Fischer Hermitian product). 
\smallskip\noindent
Given $F\in\widehat\ca O^n_\Lambda$, we shall say that $G\in\widehat\ca O^n
_\Lambda$ is {\sl a renormalized Poincar\'e-Dulac normal form} of $F$ if 
$G$ is in renormalized Poincar\'e-Dulac normal form and $G=\Phi^{-1}\circ F\circ\Phi$ for some $\Phi\in\widehat\ca O^n_I$. 

To proceed with the renormalization as explained in the introduction, we need condition \eqdd,
that is we need to check that the operator $L_{F_\mu,\Lambda}$ with $F_\mu\in\ca N^\mu$
sends $\ca H^{\nu-\mu+1}_\Lambda$ into $\ca N^\nu$. When $\Lambda$ is diagonal, we
have $\ca N^\nu=\ca H^\nu_\Lambda$ for all $\nu\ge 2$, and hence \eqdd\ follows
from Corollary~\uqua. We then have the renormalized normal form we were looking for:

\newthm Theorem \dsei: Let $\Lambda\in M_{n,n}(\C)$ be diagonal. Then each
$F\in\widehat\ca O^n_\Lambda$ admits a renormalized Poincar\'e-Dulac
normal form. More precisely, if $F=\Lambda+\sum\limits_{d\ge\mu}F_d$ is in Poincar\'e-Dulac normal form (and $F\not\equiv\Lambda$) then there exists a unique 
$\Lambda$-resonant $\Phi=I+\sum\limits_{d\ge 2}H_d\in\widehat\ca O^n_I$ such that $H_d\in(\Ker L_{F_\mu,\Lambda})^\perp$ for all $d\ge 2$ and $G=\Phi^{-1}\circ F\circ\Phi$ is in renormalized Poincar\'e-Dulac
normal form.

\pf By Proposition \foPD\ we can assume that $F$ is in Poincar\'e-Dulac
normal form. If $F\equiv\Lambda$ we are done; assume then that $F\not\equiv\Lambda$. 

First of all, by Proposition~\dquattro\ if $\Phi$ is $\Lambda$-resonant 
we have $\{\Phi^{-1}\circ F\circ\Phi\}_d=F_d$ for all $d\le\mu$. In particular, $F_\mu\in\ca H^\mu_\Lambda$; therefore, by Corollary~\uqua, $\Im L_{F_\mu,\Lambda}|_{\ca H^{\nu-\mu+1}_\Lambda}
\subseteq\ca H^\nu_\Lambda$. We then have the splittings
$$
\ca H^\nu_\Lambda=\Im L_{F_\mu,\Lambda}|_{\ca H^{\nu-\mu+1}_\Lambda}\bigoperp
(\Im L_{F_\mu,\Lambda}|_{\ca H^{\nu-\mu+1}_\Lambda})^\perp
$$
and 
$$
\ca H^{\nu-\mu+1}_\Lambda=\Ker L_{F_\mu,\Lambda}|_{\ca H^{\nu-\mu+1}_\Lambda}\bigoperp
(\Ker L_{F_\mu,\Lambda}|_{\ca H^{\nu-\mu+1}_\Lambda})^\perp\;.
$$
Hence we can find a unique $G\in(\Im L_{F_\mu,\Lambda})^\perp
\cap\ca H^{\mu+1}_\Lambda$ and a unique $H\in (\Ker L_{F_\mu,\Lambda})^\perp
\cap\ca H^{2}_\Lambda$ such that $F_{\mu+1}=G+L_{F_\mu,\Lambda}(H)$. Then 
Proposition~\dquattro\ yields
$$
\{\Phi^{-1}\circ F\circ\Phi\}_{\mu+1}=F_{\mu+1}-L_{F_\mu,\Lambda}(\{\Phi\}_2)
=G+L_{F_\mu,\Lambda}(H)-L_{F_\mu,\Lambda}(\{\Phi\}_2)\;;
$$
so to get $\{\Phi^{-1}\circ F\circ\Phi\}_{\mu+1}\in(\Im L_{F_\mu,\Lambda})^\perp
\cap\ca H^{\mu+1}_\Lambda$ with $\{\Phi\}_2\in (\Ker L_{F_\mu,\Lambda})^\perp
\cap\ca H^{2}_\Lambda$ we must necessarily take $\{\Phi\}_2=H$.

Assume, by induction, that we have uniquely determined $H_2,\ldots,H_{d-1}\in
(\Im L_{F_\mu,\Lambda})^\perp\cap\ca H_\Lambda$; in particular, this determines completely
$R_d\in\ca H^d_\Lambda$ in \eqdqua. Hence there exist a unique $G$ in $(\Im L_{F_\mu,\Lambda})^\perp
\cap\ca H^d_\Lambda$ and a unique $H\in (\Ker L_{F_\mu,\Lambda})^\perp
\cap\ca H^{d-\mu+1}_\Lambda$ such that $F_d+R_d=G+L_{F_\mu,\Lambda}(H)$. So
to get $\{\Phi^{-1}\circ F\circ\Phi\}_d\in(\Im L_{F_\mu,\Lambda})^\perp
\cap\ca H^d_\Lambda$ with $\{\Phi\}_{d-\mu+1}\in(\Ker L_{F_\mu,\Lambda})^\perp
\cap\ca H^{d-\mu+1}_\Lambda$ the 
only choice is $\{\Phi\}_{d-\mu+1}=H$, and thus $\{\Phi^{-1}\circ F\circ\Phi\}_d=G$.\qedn

%\newdef Furthermore, we shall say that
%$F$ is in {\sl Poincar\'e-Dulac normal form} if it is $\{F\}_1$-resonant.
%
%
%\newthm Corollary \dunoc: Take $\Lambda\in M_{n,n}(\C)$ and $F\in\widehat\ca O^n_\Lambda$  in Poincar\'e-Dulac normal form. If $\Phi\in\widehat\ca O^n_I$ is $\Lambda$-resonant
%then $G=\Phi^{-1}\circ F\circ\Phi$ is in Poincar\'e-Dulac normal form. Conversely, assuming
%moreover $\ca H_\Lambda\cap\Im
%L_\Lambda=(O)$, if $G$ is in Poincar\'e-Dulac normal form then $\Phi$ is
%$\Lambda$-resonant.
%
%\pf If $F$ and $\Phi$ both are $\Lambda$-resonant, it is
%clear that $G=\Phi^{-1}\circ F\circ\Phi$ is still $\Lambda$-resonant, and thus in
%Poincar\'e-Dulac normal form because $\{G\}_1=\Lambda$.
%
%Conversely,
%let $\Phi=I+\sum\limits_{d\ge 2}H_d$ be the homogeneous expansion of $\Phi$. We must
%prove by induction that $H_d\in\ca H^d_\Lambda$ for all $d\ge 2$. When $d=2$ we have
%$\{G\}_2=\{F\}_2-L_\Lambda(H_2)$; since $\{G\}_2$, $\{F\}_2\in\ca H_\Lambda$ and 
%$\ca H_\Lambda\cap\Im L_\Lambda=(O)$ by assumption, it follows that $L_\Lambda(H_2)=O$,
%that is $H_2\in\ca H_\Lambda$.
%
%Now assume, by induction, that $H_2,\ldots, H_{d-1}\in\ca H_\Lambda$. Then 
%Proposition~\dquattro.(i) yields $Q_d=O$, Proposition~\dquattro.(iv) yields $R_d\in\ca H_\Lambda$,
%and Lemma~\uqua\ yields $L_{F_\mu,\Lambda}(H_{d-\mu+1})\in\ca H_\Lambda$.
%Therefore \eqdqua\ implies $L_\Lambda(H_d)\in\ca H_\Lambda$, that is $H_d\in\ca H_\Lambda$
%as before,
%and we are done.\qedn
%
%\newthm Corollary \dduec: Take $\Lambda\in M_{n,n}(\C)$ such that 
%$\ca H_\Lambda\cap\Im L_\Lambda=(O)$. Assume that $F\in\widehat\ca O^n_\Lambda$ is formally conjugated
%to $\Lambda$. Then $\Lambda$ is the unique Poincar\'e-Dulac normal form of $F$.
%
%\pf It suffices to prove that if $F=\Lambda$ and $G=\Phi^{-1}\circ F\circ\Phi$ is in Poincar\'e-Dulac normal form, with $\Phi\in\widehat\ca O^n_I$, then $G=\Lambda$. But indeed Corollary~\dunoc\
%says that $\Phi$ is $\Lambda$-resonant, and the assertion follows.\qedn
%
%\newrem If $\Lambda$ is diagonalizable, Remark~1.1 shows that $\ca H_\Lambda\cap
%\Im L_\Lambda=(O)$. 
%
%\Nota Questi due corollari recuperano risultati tuoi nel caso diagonalizzabile, in cui l'ipotesi
%$\ca H_\Lambda\cap\Im L_\Lambda=(O)$ \`e soddisfatta. Quando $\Lambda$ non \`e
%diagonalizzabile bisogna probabilmente procedere in modo lievemente diverso, togliendo da
%$\Lambda$ la parte nilpotente, perch\'e se $\Lambda$ non \`e diagonalizzabile $\ca H_\Lambda$
%non \`e dato dai monomi risonanti rispetto agli autovalori di $\Lambda$ ma sospetto sia
%sensibilmente pi\`u piccolo. 
%
%\newrem The main consequence of \eqdqua\ is that, when $F$ is in 
%Poincar\'e-Dulac normal form, by conjugating with a $\Lambda$-resonant
%formal power series we act on the $d$-homogeneous term mainly by adding an element 
%in the image of $L_{F_\mu,\Lambda}$ restricted to the $\Lambda$-resonant homogeneous
%polynomial maps. Thus, roughly speaking, suitably choosing $H_{d-\mu+1}$ we can obtain that $\{\Phi^{-1}\circ F
%\circ\Phi\}_d$ has no components in that image. We shall now make this
%precise.

As examples of applications of this method,
in the remaining two sections we shall study cases where the usual
Poincar\'e-Dulac normal form reduces to the original map.

\smallsect 3. Examples with $\Lambda=O$

In this section we shall completely describe the renormalized normal forms obtained when $n=\mu=2$ and $\Lambda=O$, that is in the 2-dimensional quadratic superattracting case. It is worthwhile to remark that, except in a few degenerate
instances, the normal form will be expressed just in terms of two power series of {\it one} variable, and thus we shall obtain a drastic simplification of the germs.

In [A3] we 
showed that, up to a linear change of variable, we can assume that the quadratic term $F_2$ 
is of one (and only one) of the following forms:
\smallskip
\itemitem{$(\infty)$} $F_2(z,w)=(z^2,zw)$;
\itemitem{$(1_{00})$} $F_2(z,w)=(0,-z^2)$;
\itemitem{$(1_{10})$} $F_2(z,w)=\bigl(-z^2,-(z^2+zw)\bigr)$;
\itemitem{$(1_{11})$} $F_2(z,w)=\bigl(-zw,-(z^2+w^2)\bigr)$;
\itemitem{$(2_{001})$} $F_2(z,w)=(0,zw)$;
\itemitem{$(2_{011})$} $F_2(z,w)=(zw,zw+w^2)$;
\itemitem{$(2_{10\rho})$} $F_2(z,w)=\bigl(-\rho z^2,(1-\rho) zw)$, with $\rho\ne0$;
\itemitem{$(2_{11\rho})$} $F_2(z,w)=\bigl(\rho z^2+zw,(1+\rho) zw+w^2\bigr)$, with $\rho\ne0$;
\itemitem{$(3_{100})$} $F_2(z,w)=(z^2-zw,0)$;
\itemitem{$(3_{\rho10})$} $F_2(z,w)=\bigl(\rho(-z^2+zw),(1-\rho)(zw- w^2)\bigr)$, with
$\rho\ne0$,~$1$;
\itemitem{$(3_{\rho\tau1})$} $F_2(z,w)=\bigl(-\rho z^2+(1-\tau)zw,(1-\rho)
zw-\tau w^2\bigr)$, with $\rho$,~$\tau\ne0$ and $\rho+\tau\ne1$
\smallskip
\noindent (where the symbols refer to the number of characteristic directions and to their indeces;
see also [AT2]). 

%The corresponding Jacobians are:
%\itemitem{$(\infty)$} $\displaystyle\Jac F_2=\pmatrix{ 2z& 0\cr w& z\cr}$;
%\itemitem{$(1_{00})$} $\displaystyle\Jac F_2=\pmatrix{ 0& 0\cr -2z& 0\cr}$;
%\itemitem{$(1_{10})$} $\displaystyle\Jac F_2=\pmatrix{ -2z& 0\cr -2z-w& -z\cr}$;
%\itemitem{$(1_{11})$} $\displaystyle\Jac F_2=\pmatrix{ -w& -z\cr -2z&-2w \cr}$;
%\itemitem{$(2_{001})$} $\displaystyle\Jac F_2=\pmatrix{ 0& 0\cr w& z\cr}$;
%\itemitem{$(2_{011})$} $\displaystyle\Jac F_2=\pmatrix{ w& z\cr w& z+2w\cr}$;
%\itemitem{$(2_{10\rho})$} $\displaystyle\Jac F_2=\pmatrix{ -2\rho z& 0\cr (1-\rho)w& (1-\rho)z\cr}$;
%\itemitem{$(2_{11\rho})$} $\displaystyle\Jac F_2=\pmatrix{ 2\rho z+w&z \cr(1+\rho)w &
%(1+\rho)z+2w \cr}$;
%\itemitem{$(3_{100})$} $\displaystyle\Jac F_2=\pmatrix{2z-w & -z\cr 0& 0\cr}$;
%\itemitem{$(3_{\rho10})$} $\displaystyle\Jac F_2=\pmatrix{ \rho(-2z+w)&\rho z \cr 
%(1-\rho)w& (1-\rho)(z-2w)\cr}$;
%\itemitem{$(3_{\rho\tau1})$} $\displaystyle\Jac F_2=\pmatrix{-2\rho z+(1-\tau)w &(1-\tau)z \cr
%(1-\rho)w &(1-\rho)z-2\tau w \cr}$.

We shall use the standard basis $\{u_{d,j},v_{d,j}\}_{j=0,\ldots,d}$ of $\ca H^d$, where
$$
u_{d,j}=(z^jw^{d-j},0)\qquad\hbox{and}\qquad v_{d,j}=(0,z^jw^{d-j})\;,
$$
and we shall endow $\ca H^d$ with the usual Fischer scalar product, so that $\{u_{d,j},v_{d,j}\}_{j=0,\ldots,d}$ is an orthogonal basis and
$$
\|u_{d,j}\|^2=\|v_{d,j}\|^2={d\choose j}^{-1}\;.
$$
Finally, we recall that when $\Lambda=O$ the operator $L=L_{F_2,\Lambda}$ is given by
$$
L(H)=-\Jac(F_2)\cdot H\;.
$$

We shall now study separately each case.

\medbreak
\noindent$\bullet$ {\it Case $(\infty)$.}

\noindent In this case we have
$$
L(u_{d,j})=-2u_{d+1,j+1}-v_{d+1,j}\qquad\hbox{and}\qquad L(v_{d,j})=-v_{d+1,j+1}
$$
for all $d\ge 2$ and $j=0,\ldots,d$. Therefore
$$
\Im L|_{\ca H^d}=\Span{u_{d+1,2},\ldots,u_{d+1,d+1}, 2u_{d+1,1}+v_{d+1,0},v_{d+1,1},\ldots,v_{d+1,d+1}}\;,
$$
and thus
$$
(\Im L|_{\ca H^d})^\perp=\Span{u_{d+1,0},(d+1)u_{d+1,1}-2v_{d+1,0}}\;.
$$
It then follows that every formal power series of the form
$$
F(z,w)=(z^2+O_3,zw+O_3)
$$
(where $O_3$ denotes a remainder term of order at least~3)
is formally conjugated to a power series of the form
$$
G(z,w)=\bigl(z^2+\phe(w)+z\psi'(w),zw-2\psi(w)\bigr)
$$
where $\phe$, $\psi\in\C[\![\zeta]\!]$ are arbitrary power series of order at least~3. Notice that
(here and in later formulas) the appearance of the derivative (which simplifies the expression
of the normal form) is due to the fact we are using the Fischer Hermitian product; using
another Hermitian product might lead to more complicated normal
forms. 

\medbreak
\noindent$\bullet$ {\it Case $(1_{00})$.}

\noindent In this case we have
$$
L(u_{d,j})=2v_{d+1,j+1}\qquad\hbox{and}\qquad L(v_{d,j})=0
$$
for all $d\ge 2$ and $j=0,\ldots,d$. Therefore
$$
\Im L|_{\ca H^d}=\Span{v_{d+1,1},\ldots,v_{d+1,d+1}}\;,
$$
and thus
$$
(\Im L|_{\ca H^d})^\perp=\Span{u_{d+1,0},\ldots,u_{d+1,d+1},v_{d+1,0}}\;.
$$
It then follows that every formal power series of the form
$$
F(z,w)=(O_3,-z^2+O_3)
$$
is formally conjugated to a power series of the form
$$
G(z,w)=\left(\Phi(z,w),-z^2+\psi(w)\right)
$$
where $\psi\in\C[\![\zeta]\!]$ and $\Phi\in\C[\![z,w]\!]$ are arbitrary power series of
order at least~3.

\medbreak
\noindent$\bullet$ {\it Case $(1_{10})$.}

\noindent In this case we have
$$
L(u_{d,j})=2u_{d+1,j+1}+2v_{d+1,j+1}+v_{d+1,j}\qquad\hbox{and}\qquad L(v_{d,j})=v_{d+1,j+1}
$$
for all $d\ge 2$ and $j=0,\ldots,d$. Therefore
$$
\Im L|_{\ca H^d}=\Span{2u_{d+1,1}+v_{d+1,0},u_{d+1,2},\ldots,u_{d+1,d+1},v_{d+1,1},\ldots,v_{d+1,d+1}}\;,
$$
and thus
$$
(\Im L|_{\ca H^d})^\perp=\Span{u_{d+1,0},(d+1)u_{d+1,1}-2v_{d+1,0}}\;.
$$
It then follows that every formal power series of the form
$$
F(z,w)=(-z^2+O_3,-z^2-zw+O_3)
$$
is formally conjugated to a power series of the form
$$
G(z,w)=\bigl(-z^2+\phe(w)+z\psi'(w),-z^2-zw-2\psi(w)\bigr)
$$
where $\phe$,~$\psi\in\C[\![\zeta]\!]$ are arbitrary power series of order at least~3.

\medbreak
\noindent$\bullet$ {\it Case $(1_{11})$.}

\noindent In this case we have
$$
L(u_{d,j})=u_{d+1,j}+2v_{d+1,j+1}\qquad\hbox{and}\qquad L(v_{d,j})=u_{d+1,j+1}+2v_{d+1,j}
$$
for all $d\ge 2$ and $j=0,\ldots,d$. It follows that 
$$
\eqalign{
\Im L|_{\ca H^d}=\hbox{\rm Span}(&u_{d+1,0}-u_{d+1,2},\ldots,u_{d+1,d-1}-u_{d+1,d+1},\cr
&\quad v_{d+1,2}-v_{d+1,0},
\ldots,v_{d+1,d+1}-v_{d+1,d-1},u_{d+1,0}+2v_{d+1,1},u_{d+1,1}+2v_{d+1,0})\;,\cr}
$$
and a few computations yield
$$
\eqalign{
(\Im L|_{\ca H^d})^\perp&=\Span{\sum_{j=0}^{d+1}{d+1\choose j}(v_{d+1,j}-2u_{d+1,j}),
\sum_{j=0}^{d+1}(-1)^j{d+1\choose j}(v_{d+1,j}+2u_{d+1,j})}\cr
&=\Span{\bigl(-2(z+w)^{d+1},(z+w)^{d+1}\bigr),\bigl(2(w-z)^{d+1},(w-z)^{d+1}\bigr)}\cr}\;.
$$
It then follows that every formal germ of the form
$$
F(z,w)=(-zw+O_3,-z^2-w^2+O_3)
$$
is formally conjugated to a germ of the form
$$
G(z,w)=\bigl(-zw-2\phe(z+w)+2\psi(w-z),
-z^2-w^2+\phe(z+w)+
\psi(w-z)\bigr)
$$
where $\phe$,~$\psi\in\C[\![\zeta]\!]$ are arbitrary power series of order at least~3. Again, the fact that the normal form is expressed in terms of power series evaluated in $z+w$ and $z-w$
is due to the fact we are using the Fischer Hermitian product.

\medbreak
\noindent$\bullet$ {\it Case $(2_{001})$.}

\noindent In this case we have
$$
L(u_{d,j})=-v_{d+1,j}\qquad\hbox{and}\qquad L(v_{d,j})=-v_{d+1,j+1}
$$
for all $d\ge 2$ and $j=0,\ldots,d$. It follows that 
$$
\Im L|_{\ca H^d}=\Span{v_{d+1,0},\ldots,v_{d+1,d+1}}
$$
and hence
$$
(\Im L|_{\ca H^d})^\perp=\Span{u_{d+1,0},\ldots,u_{d+1,d+1}}\;.
$$
It then follows that every formal germ of the form
$$
F(z,w)=(O_3,zw+O_3)
$$
is formally conjugated to a germ of the form
$$
G(z,w)=\bigl(\Phi(z,w),zw\bigr)
$$
where $\Phi\in\C[\![z,w]\!]$ is a power series of order at least three.

\medbreak
\noindent$\bullet$ {\it Case $(2_{011})$.}

\noindent In this case we have
$$
L(u_{d,j})=-u_{d+1,j}-v_{d+1,j}\qquad\hbox{and}\qquad L(v_{d,j})=-u_{d+1,j+1}-2v_{d+1,j}
-v_{d+1,j+1}
$$
for all $d\ge 2$ and $j=0,\ldots,d$. It follows that 
$$
\eqalign{
\Im L|_{\ca H^d}&=\hbox{\rm Span}(u_{d+1,0},\ldots,u_{d+1,d-1},v_{d+1,0},\ldots,v_{d+1,d-1},\cr
&\qquad\qquad u_{d+1,d}+v_{d+1,d},u_{d+1,d+1}+v_{d+1,d+1}+2v_{d+1,d})\;,\cr}
$$
and hence
$$
(\Im L|_{\ca H^d})^\perp=\Span{(d+1) u_{d+1,d}- (d+1) v_{d+1,d}+2v_{d+1,d+1},u_{d+1,d+1}-v_{d+1,d+1}}\;.
$$
It then follows that every formal germ of the form
$$
F(z,w)=(zw+O_3,zw+w^2+O_3)
$$
is formally conjugated to a germ of the form
$$
G(z,w)=\bigl( zw + w\phe'(z) + \psi(z),
zw + w^2 + 2\phe(z) - w\phe'(z) - \psi(z)\bigr)\;,
$$
where $\phe$, $\psi\in\C[\![\zeta]\!]$ are arbitrary power series of order at least~3.

\medbreak
\noindent$\bullet$ {\it Case $(2_{10\rho})$.}

\noindent In this case we have
$$
L(u_{d,j})=2\rho u_{d+1,j+1}+(\rho-1)v_{d+1,j}\qquad\hbox{and}\qquad L(v_{d,j})=(\rho-1)v_{d+1,j+1}$$
for all $d\ge 2$ and $j=0,\ldots,d$. We clearly have two subcases to consider.

If $\rho=1$ then
$$
\Im L|_{\ca H^d}=\Span{u_{d+1,1},\ldots,u_{d+1,d+1}}\;,
$$
and hence
$$
(\Im L|_{\ca H^d})^\perp=\Span{u_{d+1,0},v_{d+1,0},\ldots,v_{d+1,d+1}}\;.
$$
It then follows that every formal germ of the form
$$
F(z,w)=(-z^2+O_3,O_3)
$$
is formally conjugated to a germ of the form
$$
G(z,w)=\bigl(-z^2+\psi(w),\Phi(z,w)\bigr)\;,
$$
where $\psi\in\C[\![\zeta]\!]$ and $\Phi\in\C[\![z,w]\!]$ are arbitrary power series of order at least~3.

If instead $\rho\ne 1$ (recalling that $\rho\ne0$ too) then
$$
\Im L|_{\ca H^d}=\Span{2\rho u_{d+1,1} + (\rho - 1) v_{d+1,0}, u_{d+1,2},\ldots,u_{d+1,d+1},v_{d+1,1},\ldots,v_{d+1,d+1}}\;,
$$
and hence
$$
(\Im L|_{\ca H^d})^\perp=\Span{u_{d+1,0},(\rho-1)(d+1) u_{d+1,1} - 2\rho v_{d+1,0}}\;.
$$
It then follows that every formal germ of the form
$$
F(z,w)=\bigl(-\rho z^2+O_3,(1-\rho)zw+O_3\bigr)
$$
with $\rho\ne 0$,~$1$ is formally conjugated to a germ of the form
$$
G(z,w)=\bigl(- \rho z^2+ (\rho -1) z\phe'(w)+ \psi(w),(1-\rho)zw - 2\rho\phe(z)\bigr)\;,
$$
where $\phe$,~$\psi\in\C[\![\zeta]\!]$ are arbitrary power series of order at least~3.

\medbreak
\noindent$\bullet$ {\it Case $(2_{11\rho})$.}

\noindent In this case we have
$$
\cases{
L(u_{d,j})=-2\rho u_{d+1,j+1}-u_{d+1,j}-(1+\rho)v_{d+1,j}\cr
L(v_{d,j})=
-u_{d+1,j+1}-2v_{d+1,j}-(1+\rho)v_{d+1,j+1}\cr}
\neweq\eqtuno
$$
for all $d\ge 2$ and $j=0,\ldots,d$. We clearly have two subcases to consider.

If $\rho=-1$ then
$$
\Im L|_{\ca H^d}=\Span{u_{d+1,0}-2u_{d+1,1},\ldots,u_{d+1,d}-2u_{d+1,d+1},
u_{d+1,1}+2v_{d+1,0},\ldots,u_{d+1,d}+2v_{d+1,d}}\;,
$$
and hence
$$
\eqalign{
(\Im L|_{\ca H^d})^\perp&=\Span{\sum_{j=0}^{d+1}{d+1\choose j}{1\over 2^j}(u_{d+1,j}-{1\over 4}
v_{d+1,j}),v_{d+1,d+1}}\cr
&=\Span{\left(\left({\textstyle{{z\over 2}}}+w\right)^{d+1},-{1\over 4}\left({\textstyle{{z\over 2}}}+w\right)^{d+1}
\right),(0,z^{d+1})}\;.\cr}
$$
It then follows that every formal germ of the form
$$
F(z,w)=(-z^2+zw+O_3,w^2+O_3)
$$
is formally conjugated to a germ of the form
$$
G(z,w)=\left(-z^2+zw+\phe({\textstyle{{z\over 2}}}+w),
w^2- {1\over 4}\phe({\textstyle{{z\over 2}}}+w)+\psi(z)\right)\;,
$$
where $\phe$,~$\psi\in\C[\![\zeta]\!]$ are arbitrary power series of order at least~3.

If instead $\rho\ne -1$ (recalling that $\rho\ne0$ too) then a basis of $\Im L|_{\ca H^d}$
is given by the vectors listed in \eqtuno, and a computation shows that $(\Im L|_{\ca H^d})^\perp$
is given by homogeneous maps of the form
$$
\sum_{j=0}^{d+1}(a_j u_{d+1,j}+b_j v_{d+1,j})
$$
where the coefficients $a_j$, $b_j$ satisfy the following relations:
$$
\cases{\displaystyle c_jb_j=-{2\over1+\rho}c_{j-1}b_{j-1}-{1\over\rho(1+\rho)}c_{j-2}b_{j-2}&for $j=2,\ldots,d+1$,\cr
\noalign{\smallskip}
\displaystyle c_ja_j={1\over\rho}c_{j-2}b_{j-2}&for $j=2,\ldots,d+1$,\cr
\noalign{\smallskip}
\displaystyle a_0=(3\rho-1)b_0+2{\rho(1+\rho)\over d+1}b_1\;,\cr
\noalign{\smallskip}
\displaystyle a_1=-2(d+1)b_0-(1+\rho)b_1\;,\cr}
$$
where $c_j^{-1}={d+1\choose j}$
and $b_0$, $b_1\in\C$ are arbitrary. Solving this recurrence equation one gets
$$
b_j={1\over2\sqrt{-\rho}}{d+1\choose j}\left[{\rho(1+\rho)\over d+1}(m_\rho^j-n_\rho^j)b_1
+\bigl(\rho(m_\rho^j-n_\rho^j)+\sqrt{-\rho}(m_\rho^j+n_\rho^j)\bigr)b_0\right]\;,
$$
where $\sqrt{-\rho}$ is any square root of $-\rho$, and
$$
m_\rho={\sqrt{-\rho}-\rho\over\rho(1+\rho)}\;,\qquad n_\rho=-{\sqrt{-\rho}+\rho\over\rho(1+\rho)}\;.
$$
It follows that the renormalized normal form of a formal germ of the form
$$
F(z,w)=\bigl(\rho z^2+zw+O_3,(1+\rho)zw+w^2+O_3\bigr)
$$
with $\rho\ne 0$,~$-1$ is
$$
\eqalign{
G(z,w)=&\left(\rho z^2+zw+{1\over\rho}\left[{1-\sqrt{-\rho}\over 2m_\rho^2}\phe(m_\rho z+w)
+{1+\sqrt{-\rho}\over 2n_\rho^2}\phe(n_\rho z+w)\right]\right.\cr
&\phantom{\biggl(\rho z^2+zw\,}
+{1+\rho\over2\sqrt{-\rho}}\left(
{1\over m_\rho^2}\psi(m_\rho z+w)-{1\over n_\rho^2}\psi(n_\rho z+w)\right),\cr
&\quad(1+\rho)zw+w^2+ {1-\sqrt{-\rho}\over2}\phe(m_\rho z+w)+{1+\sqrt{-\rho}\over2}\phe(n_\rho z+w)\cr
&\phantom{\biggl((1+\rho)zw+w^2\;}+\left.{\rho(1+\rho)\over2\sqrt{-\rho}}\bigl(\psi(m_\rho z+w)-\psi(n_\rho z+w)\bigr)
\right)\cr}
$$ 
where $\phe$,~$\psi\in\C[\![\zeta]\!]$ are power series of order at least~3.

\medbreak
\noindent$\bullet$ {\it Case $(3_{100})$.}

\noindent In this case we have
$$
L(u_{d,j})=u_{d+1,j}-2u_{d+1,j+1}\qquad\hbox{and}\qquad L(v_{d,j})=u_{d+1,j+1}
$$
for all $d\ge 2$ and $j=0,\ldots,d$. It follows that 
$$
\Im L|_{\ca H^d}=\Span{u_{d+1,0},\ldots,u_{d+1,d+1}}
$$
and hence
$$
(\Im L|_{\ca H^d})^\perp=\Span{v_{d+1,0},\ldots,v_{d+1,d+1}}\;.
$$
It then follows that every formal germ of the form
$$
F(z,w)=(z^2-zw+O_3,O_3)
$$
is formally conjugated to a germ of the form
$$
G(z,w)=\bigl(z^2-zw,\Phi(z,w)\bigr)\;,
$$
where $\Phi\in\C[\![z,w]\!]$ is a power series of order at least~3.

\medbreak
\noindent$\bullet$ {\it Case $(3_{\rho10})$.}

\noindent In this case we have
$$
\cases{
L(u_{d,j})=\rho(2u_{d+1,j+1}-u_{d+1,j})+(\rho-1)v_{d+1,j}\cr
L(v_{d,j})=-\rho u_{d+1,j+1}+(\rho-1)(v_{d+1,j+1}-2v_{d+1,j})\cr}
\neweq\eqtdue
$$
for all $d\ge 2$ and $j=0,\ldots,d$. Then a basis of $\Im L|_{\ca H^d}$ is given by the 
homogeneous maps listed in \eqtdue, and a computation shows that $(\Im L|_{\ca H^d})^\perp$
is given by homogeneous maps of the form
$$
\sum_{j=0}^{d+1}(a_j u_{d+1,j}+b_j v_{d+1,j})
$$
where the coefficients $a_j$, $b_j$ satisfy the following relations:
$$
\cases{\displaystyle c_{j+1}a_{j+1}={\rho-1\over\rho}(c_{j+1}b_{j+1}-2c_jb_j)&for $j=0,\ldots,d$,\cr
\noalign{\smallskip}
\displaystyle c_{j+1}b_{j+1}=2c_jb_j-c_{j-1}b_{j-1}&for $j=1,\ldots,d$,\cr
\noalign{\smallskip}
\displaystyle c_0a_0=2c_1a_1+{\rho-1\over \rho}c_0b_0\;,\cr}
$$
where $c_j^{-1}={d+1\choose j}$ and $b_0$, $b_1\in\C$ are arbitrary. Solving this recurrence
equation we find
$$
\cases{
b_j={d+1\choose j}\left[{j\over d+1}b_1-(j-1)b_0\right]&
for $j=0,\ldots,d+1$,\cr
a_j={\rho-1\over \rho}{d+1\choose j}\left[{2-j\over d+1}b_1+(j-3)b_0
\right]&for $j=0,\ldots,d+1$,\cr}
$$
where $b_0$, $b_1\in\C$ are arbitrary. So every formal germ of the form
$$
F(z,w)=\bigl(\rho (-z^2+zw)+O_3,(1-\rho)(zw-w^2)+O_3\bigr)
$$
with $\rho\ne 0$,~$1$ is formally conjugated to a germ of the form
$$
\eqalign{
G(z,w)=&\left(\rho(-z^2+zw)+z{\de\over\de z}\bigl[\phe(z+w)+\psi(z+w)\bigr]-\phe(z+w),\right.\cr
&\left.\quad(1-\rho)(zw-w^2)+{\rho-1\over\rho}\left(z{\de\over\de z}\bigl[\phe(z+w)-\psi(z+w)\bigr]
-3\phe(z+w)+2\psi(z+w)\right)
\right)\cr}
$$ 
where $\phe$,~$\psi\in\C[\![\zeta]\!]$ are power series of order at least~3.

\medbreak
\noindent$\bullet$ {\it Case $(3_{\rho\tau1})$.}

\noindent In this case we have
$$
L(u_{d,j})=(\tau-1)u_{d+1,j}+2\rho u_{d+1,j+1}+(\rho-1)v_{d+1,j}
$$
and
$$  
L(v_{d,j})=(\tau-1)u_{d+1,j+1}+2\tau v_{d+1,j}+(\rho-1)v_{d+1,j+1}
$$
for all $d\ge 2$ and $j=0,\ldots,d$. As before, we have a few subcases to consider.

Assume first $\rho=\tau=1$. Then
$$
\Im L|_{\ca H^d}=\Span{u_{d+1,1},\ldots,u_{d+1,d+1},v_{d+1,0},\ldots,v_{d+1,d}}\;;
$$
hence
$$
(\Im L|_{\ca H^d})^\perp=\Span{u_{d+1,0},v_{d+1,d+1}}\;,
$$
It then follows that every formal germ of the form
$$
F(z,w)=(-z^2+O_3,-w^2+O_3)
$$
is formally conjugated to a germ of the form
$$
G(z,w)=\bigl(-z^2+\phe(w),-w^2+\psi(z)\bigr)\;,
$$
where $\phe$,~$\psi\in\C[\![z,w]\!]$ are arbitrary power series of order at least~3.

Assume now $\rho\ne 1$. Then a computation shows that $(\Im L|_{\ca H^d})^\perp$
is given by homogeneous maps of the form
$$
\sum_{j=0}^{d+1}(a_j u_{d+1,j}+b_j v_{d+1,j})
$$
where the coefficients $a_j$, $b_j$ satisfy the following relations:
$$
\cases{\displaystyle c_{j+1}a_{j+1}={\tau\over\rho}c_{j-1}b_{j-1}&for $j=1,\ldots,d$,\cr
\noalign{\smallskip}
\displaystyle c_{j+1}b_{j+1}=-{2\tau\over\rho-1}c_jb_j-{\tau(\tau-1)\over\rho(\rho-1)}c_{j-1}b_{j-1}&for $j=1,\ldots,d$,\cr
\noalign{\smallskip}
\displaystyle (\tau-1)c_1a_1+(\rho-1)c_1b_1+2\tau c_0b_0=0\;,\cr
\displaystyle (\tau-1)c_0a_0+(\rho-1)c_0b_0+2\rho c_1a_1=0\;,\cr}
\neweq\eqttre
$$
where $c_j^{-1}={d+1\choose j}$ and $b_0$, $b_1\in\C$ are arbitrary. 

When $\tau=1$ conditions \eqttre\ reduce to
$$
\cases{\displaystyle c_{j+1}a_{j+1}={1\over\rho}c_{j-1}b_{j-1}&for $j=1,\ldots,d$,\cr
\noalign{\smallskip}
\displaystyle c_{j+1}b_{j+1}=-{2\over\rho-1}c_jb_j&for $j=1,\ldots,d$,\cr
\noalign{\smallskip}
\displaystyle (\rho-1)c_1b_1+2 c_0b_0=0\;,\cr
\displaystyle (\rho-1)c_0b_0+2\rho c_1a_1=0\;,\cr}
$$
whose solution is
$$
\cases{
\displaystyle a_j={d+1\choose j}{1\over\rho}\left({2\over 1-\rho}\right)^{j-2}b_0&for $j=1,\ldots,d+1$,\cr
\noalign{\smallskip}
\displaystyle b_j={d+1\choose j}\left({2\over1-\rho}\right)^j b_0&for $j=0,\ldots, d+1$,\cr}
$$
where $a_0$, $b_0\in\C$ are arbitrary. Therefore
$$
(\Im L|_{\ca H^d})^\perp=\Span{(w^{d+1},0),\left({(1-\rho)^2\over4\rho}\left({2\over1-\rho}z+w
\right)^{d+1}, \left({2\over1-\rho}z+w\right)^{d+1}\right)}\;,
$$
and thus every formal germ of the form
$$
F(z,w)=\bigl(-\rho z^2+O_3,(1-\rho)zw- w^2+O_3\bigr)
$$
with $\rho\ne 1$ is formally conjugated to a germ of the form
$$
G(z,w)=\left(-\rho z^2+\phe(w)+{(1-\rho)^2\over4\rho}\psi\left({2\over1-\rho}z+w\right),
(1-\rho)zw-w^2+\psi\left(
{2\over1-\rho}z+w\right)\right)\;,
$$
where $\phe$,~$\psi\in\C[\![\zeta]\!]$ are arbitrary power series of order at least~3.

The case $\rho=1$ and $\tau\ne 1$ is treated in the same way; we get that
every formal germ of the form
$$
F(z,w)=\bigl(- z^2+(1-\tau)zw+O_3,-\tau w^2+O_3\bigr)
$$
with $\tau\ne 1$ is formally conjugated to a germ of the form
$$
G(z,w)=\left(- z^2+(1-\tau)zw+\psi\left({1-\tau\over 2}z+w\right),
-\tau w^2+\phe(z)+{(1-\tau)^2\over 4\tau}\psi\left(
{1-\tau\over 2}z+w\right)\right)\;,
$$
where $\phe$,~$\psi\in\C[\![\zeta]\!]$ are arbitrary power series of order at least~3.

Finally assume $\rho$,~$\tau\ne 1$. Solving the recurrence
equation \eqttre\ we find
$$
\eqalign{
b_j={1\over2\sqrt{\rho\tau(\rho+\tau-1)}}{d+1\choose j}&\left[{\rho(\rho-1)\over d+1}(m_{\rho,\tau}^j-n_{\rho,\tau}^j)b_1\right.\cr
&\quad+\bigl(\rho\tau(m_{\rho,\tau}^j-n_{\rho,\tau}^j)+\sqrt{\rho\tau(\rho+\tau-1)}(m_{\rho,\tau}^j+n_{\rho,\tau}^j)\bigr)b_0\biggr]\;,\cr}
$$
for $j=0,\ldots,d+1$,
where $\sqrt{\rho\tau(\rho+\tau-1)}$ is any square root of $\rho\tau(\rho+\tau-1)$, and
$$
m_{\rho,\tau}={\sqrt{\rho\tau(\rho+\tau-1)}-\rho\tau\over\rho(\rho-1)}\;,\qquad n_{\rho,\tau}
=-{\sqrt{\rho\tau(\rho+\tau-1)}+\rho\tau\over\rho(\rho-1)}\;.
$$
Moreover, from \eqttre\ we also get
$$
\eqalign{
a_j={\tau\over2\rho\sqrt{\rho\tau(\rho+\tau-1)}}{d+1\choose j}&\left[{\rho(\rho-1)\over d+1}(m_{\rho,\tau}^{j-2}-n_{\rho,\tau}^{j-2})b_1\right.\cr
&\quad+\bigl(\rho\tau(m_{\rho,\tau}^{j-2}-n_{\rho,\tau}^{j-2})+\sqrt{\rho\tau(\rho+\tau-1)}(m_{\rho,\tau}^{j-2}+n_{\rho,\tau}^{j-2})\bigr)b_0\biggr]\;,\cr}
$$
again for $j=0,\ldots,d+1$.
It follows that the renormalized normal form of a formal germ of the form
$$
F(z,w)=\bigl(-\rho z^2+(1-\tau)zw+O_3,(1-\rho)zw-\tau w^2+O_3\bigr)
$$
with $\rho$, $\tau\ne 0$,~1 and $\rho+\tau\ne 1$, is
$$
\eqalign{
G(z,w)=&\left(-\rho z^2+(1-\tau)zw
+{\tau\over\rho}\left[{\sqrt{\rho+\tau-1}+\sqrt{\rho\tau}\over 2m_{\rho,\tau}^2}\phe(m_{\rho,\tau}z+w)
\right.\right.\cr
&\phantom{-\rho z^2+(1-\tau)zw+{\tau\over\rho}\biggl[\quad}+{\sqrt{\rho+\tau-1}-\sqrt{\rho\tau}\over 2n_{\rho,\tau}^2}\phe(n_{\rho,\tau}z+w)\cr
&\phantom{-\rho z^2+(1-\tau)zw+{\tau\over\rho}\biggl[\quad}\left.+
{1\over m_{\rho,\tau}^2}\psi(m_{\rho,\tau}z+w)-{1\over n_{\rho,\tau}^2}\psi(n_{\rho,\tau}z+w)\right],
\cr
&\quad(1-\rho)zw-\tau w^2+{\sqrt{\rho+\tau-1}+\sqrt{\rho\tau}\over 2}\phe(m_{\rho,\tau}z+w)\cr
&\phantom{\quad(1-\rho)zw-\tau w^2\,}
+{\sqrt{\rho+\tau-1}-\sqrt{\rho\tau}\over 2}\phe(n_{\rho,\tau}z+w)\cr
&\phantom{\quad(1-\rho)zw-\tau w^2\,}+\psi(m_{\rho,\tau}z+w)-\psi(n_{\rho,\tau}z+w)
\Biggr)\;,\cr}
$$ 
where the square roots of $\rho\tau$ and of $\rho+\tau-1$ are chosen so that their product is
equal to the previously chosen square root of $\rho\tau(\rho+\tau-1)$, and $\phe$,~$\psi\in\C[\![\zeta]\!]$ are power series of order at least~3.

\smallsect 4. Examples with $\Lambda=I$

In this section we shall assume $n=\mu=2$ and $\Lambda=I$, that is we shall be interested
in 2-dimensional germs tangent to the identity of order~2. We shall keep using the notations introduced 
in the previous section. It should be recall that in his monumental work [\'E1] (see [\'E2] for
a survey) \'Ecalle studied the formal classification of germs tangent to the identity in dimension~$n$, giving a complete set of formal invariants for germs satisfying a generic condition:
the existence of at least one non-degenerate characteristic direction (an eigenradius, in
\'Ecalle's terminology). A {\sl characteristic direction} of a germ tangent to the identity $F$ is
a non-zero direction $v$ such that $F_\mu(v)=\lambda v$ for some $\lambda\in\C$, where
$F_\mu$ is the first (nonlinear) non-vanishing term in the homogeneous expansion of~$F$. The characteristic
direction $v$ is {\sl degenerate} if $\lambda=0$.

For this reason, we decided to discuss here the cases {\it without} non-degenerate
characteristic directions, that is the cases $(1_{00})$, $(1_{10})$ and $(2_{001})$, that cannot be
dealt with \'Ecalle's methods. Furthermore, we shall also study the somewhat special case
$(\infty)$, where all directions are characteristic; and we shall examine in detail case $(2_{10\rho})$, 
where interesting second-order resonance phenomena appear.

When $\Lambda=I$ the operator $L=L_{F_2,\Lambda}$ is given by
$$
L(H)=\Jac(H)\cdot F_2-\Jac(F_2)\cdot H\;.
$$
%In particular we shall need the following computation:
%$$
%\Jac(u_{d,j})=\pmatrix{j z^{j-1}w^{d-j}&(d-j)z^j w^{d-j-1}\cr 0&0\cr}\>\hbox{and}\>
%\Jac(v_{d,j})=\pmatrix{0& 0\cr j z^{j-1}w^{d-j}&(d-j)z^j w^{d-j-1}\cr}\;.
%$$

\medbreak
\noindent$\bullet$ {\it Case $(\infty)$.}

\noindent In this case we have
$$
L(u_{d,j})=(d-2)u_{d+1,j+1}-v_{d+1,j}\qquad\hbox{and}\qquad L(v_{d,j})=(d-1)v_{d+1,j+1}
$$
for all $d\ge 2$ and $j=0,\ldots,d$. Therefore
$$
\Im L|_{\ca H^d}=
\cases{\Span{u_{d+1,2},\ldots,u_{d+1,d+1}, (d-2)u_{d+1,1}-v_{d+1,0},v_{d+1,1},\ldots,v_{d+1,d+1}}&for $d>2$,\cr
\Span{v_{3,0},\ldots,v_{3,3}}&for $d=2$.\cr}
$$
Thus
$$
(\Im L|_{\ca H^d})^\perp=
\cases{\Span{u_{d+1,0},(d+1)u_{d+1,1}+(d-2)v_{d+1,0}}&for $d>2$,\cr
\Span{u_{3,0},\ldots,u_{3,3}}&for $d=2$.\cr}
$$
It then follows that every formal power series of the form
$$
F(z,w)=(z+z^2+O_3,w+zw+O_3)
$$
is formally conjugated to a power series of the form
$$
G(z,w)=\left(z+z^2+a_0z^3+a_1z^2w+a_2 zw^2+ \phe(w)+z\psi'(w),zw+w\psi'(w)-3\psi(w)\right)
$$
where $\phe\in\C[\![\zeta]\!]$ is an arbitrary power series of order at least~3, $\psi\in\C[\![\zeta]\!]$ is an arbitrary power series of order at least~4 and $a_0$,~$a_1$,~$a_2\in\C$.

\medbreak
\noindent$\bullet$ {\it Case $(1_{00})$.}

\noindent In this case we have
$$
L(u_{d,j})=(j-d)u_{d+1,j+2}+2v_{d+1,j+1}\qquad\hbox{and}\qquad L(v_{d,j})=(j-d)v_{d+1,j+2}
$$
for all $d\ge 2$ and $j=0,\ldots,d$. Therefore
$$
\Im L|_{\ca H^d}=\Span{2v_{d+1,1}-du_{d+1,2}, u_{d+1,3},\ldots,u_{d+1,d+1},v_{d+1,2},\ldots,v_{d+1,d+1}}\;,
$$
and thus
$$
(\Im L|_{\ca H^d})^\perp=\Span{u_{d+1,0},u_{d+1,1},v_{d+1,0},u_{d+1,2}+v_{d+1,1}}\;.
$$
It then follows that every formal power series of the form
$$
F(z,w)=(z+O_3,w-z^2+O_3)
$$
is formally conjugated to a power series of the form
$$
G(z,w)=\left(z+w\phe_1(w)+z\phe_2(w)+z^2\psi(w),w-z^2+w\phe_3(w)+zw\psi(w)\right)\;,
$$
where $\phe_1$, $\phe_2$, $\phe_3\in\C[\![\zeta]\!]$ are arbitrary power series of order at least~2, and $\psi\in\C[\![\zeta]\!]$ is an arbitrary power series of
order at least~1.

\medbreak
\noindent$\bullet$ {\it Case $(1_{10})$.}

\noindent In this case we have
$$
L(u_{d,j})=(2-d)u_{d+1,j+1}-(d-j)u_{d+1,j+2}+2v_{d+1,j+1}+v_{d+1,j}
$$
and
$$
L(v_{d,j})=(1-d)v_{d+1,j+1}-(d-j)v_{d+1,j+2}
$$
for all $d\ge 2$ and $j=0,\ldots,d$. Therefore
$$
\Im L|_{\ca H^d}=
\cases{\Span{(2-d)u_{d+1,1}+v_{d+1,0},u_{d+1,2},\ldots,u_{d+1,d+1},v_{d+1,1},\ldots,v_{d+1,d+1}}&for $d>2$,\cr
\Span{v_{3,0}-2u_{3,2},u_{3,3},v_{3,1},v_{3,2},v_{3,3}}&for $d=2$,\cr}
$$
and thus
$$
(\Im L|_{\ca H^d})^\perp=
\cases{\Span{u_{d+1,0},(d+1)u_{d+1,1}+(d-2)v_{d+1,0}}&for $d>2$,\cr
\Span{u_{3,0},u_{3,1},3u_{3,2} + 2v_{3,0}}&for $d=2$.\cr}
$$
It then follows that every formal power series of the form
$$
F(z,w)=(z-z^2+O_3,w-z^2-zw+O_3)
$$
is formally conjugated to a power series of the form
$$
{
G(z,w)=\bigl(z-z^2+\phe(w)+a_1zw^2+3a_2z^2w+z\psi'(w), w-z^2-zw+2a_2w^3+w\psi'(w)-3\psi(w)\bigr)\;,}
$$
where $\phe\in\C[\![\zeta]\!]$ is an arbitrary power series of order at least~3, $\psi\in\C[\![\zeta]\!]$ is an arbitrary power series of order at least~4, and $a_1$,~$a_2\in\C$.

%\medbreak
%\noindent$\bullet$ {\it Case $(1_{11})$.}
%
%\noindent In this case we have
%$$
%L(u_{d,j})=(1-d)u_{d+1,j}-(d-j)u_{d+1,j+2}+2v_{d+1,j+1}
%$$
%and
%$$
%L(v_{d,j})=u_{d+1,j+1}+(2-d)v_{d+1,j}-(d-j)v_{d+1,j+2}
%$$
%for all $d\ge 2$ and $j=0,\ldots,d$. It follows that ???
%$$
%\eqalign{
%\Im L|_{\ca H^d}=\hbox{\rm Span}(&u_{d+1,0}-u_{d+1,2},\ldots,u_{d+1,d-1}-u_{d+1,d+1},\cr
%&\quad v_{d+1,2}-v_{d+1,0},
%\ldots,v_{d+1,d+1}-v_{d+1,d-1},u_{d+1,0}+2v_{d+1,1},u_{d+1,1}+2v_{d+1,0})\;,\cr}
%$$
%and a few computations yield
%$$
%\eqalign{
%(\Im L|_{\ca H^d})^\perp&=\Span{\sum_{j=0}^{d+1}{d+1\choose j}(v_{d+1,j}-2u_{d+1,j}),
%\sum_{j=0}^{d+1}(-1)^j{d+1\choose j}(v_{d+1,j}+2u_{d+1,j})}\cr
%&=\Span{\bigl(-2(z+w)^{d+1},(z+w)^{d+1}\bigr),\bigl(2(w-z)^{d+1},(w-z)^{d+1}\bigr)}\cr}\;.
%$$
%It then follows that every formal germ of the form
%$$
%F(z,w)=(-zw+O_3,-z^2-w^2+O_3)
%$$
%is formally conjugated to a germ of the form
%$$
%G(z,w)=\bigl(-zw-2\phe(z+w)+2\psi(w-z),
%-z^2-w^2+\phe(z+w)+
%\psi(w-z)\bigr)
%$$
%where $\phe$,~$\psi\in\C[\![w]\!]$ are arbitrary power series of order at least~3.

\medbreak
\noindent$\bullet$ {\it Case $(2_{001})$.}

\noindent In this case we have
$$
L(u_{d,j})=(d-j)u_{d+1,j+1}-v_{d+1,j}\qquad\hbox{and}\qquad L(v_{d,j})=(d-j-1)v_{d+1,j+1}
$$
for all $d\ge 2$ and $j=0,\ldots,d$. It follows that 
$$
\Im L|_{\ca H^d}=\Span{du_{d+1,1}-v_{d+1,0},u_{d+1,2},\ldots,u_{d+1,d},v_{d+1,1},\ldots,v_{d+1,d+1}}
$$
and hence
$$
(\Im L|_{\ca H^d})^\perp=\Span{u_{d+1,0},u_{d+1,d+1},(d+1)u_{d+1,1}+dv_{d+1,0}}\;.
$$
It then follows that every formal germ of the form
$$
F(z,w)=(z+O_3,w+zw+O_3)
$$
is formally conjugated to a germ of the form
$$
G(z,w)=\bigl(z+\phe_1(z)+\phe_2(w)+z\psi'(w),zw+w\psi'(w)-\psi(w)\bigr)
$$
where $\phe_1$, $\phe_2$, $\psi\in\C[\![\zeta]\!]$ are arbitrary power series of order at least~3.

%\medbreak
%\noindent$\bullet$ {\it Case $(2_{011})$.}
%
%\noindent In this case we have
%$$
%L(u_{d,j})=(d-1)u_{d+1,j}+(d-j)u_{d+1,j+1}-v_{d+1,j}
%$$
%and
%$$
%L(v_{d,j})=-u_{d+1,j+1}+(d-2)v_{d+1,j}+(d-j-1)v_{d+1,j+1}
%$$
%for all $d\ge 2$ and $j=0,\ldots,d$. It follows that ???
%$$
%\eqalign{
%\Im L|_{\ca H^d}&=\hbox{\rm Span}(u_{d+1,0},\ldots,u_{d+1,d-1},v_{d+1,0},\ldots,v_{d+1,d-1},\cr
%&\qquad\qquad u_{d+1,d}+v_{d+1,d},u_{d+1,d+1}+v_{d+1,d+1}+2v_{d+1,d})\;,\cr}
%$$
%and hence
%$$
%(\Im L|_{\ca H^d})^\perp=\Span{du_{d+1,d}-dv_{d+1,d}+2v_{d+1,d+1},u_{d+1,d+1}-v_{d+1,d+1}}\;.
%$$
%It then follows that every formal germ of the form
%$$
%F(z,w)=(zw+O_3,zw+w^2+O_3)
%$$
%is formally conjugated to a germ of the form
%$$
%G(z,w)=\bigl(zw+zw\phe'(z)+z\psi(z),
%zw+w^2+2z\phe(z)-zw\phe'(z)-z\psi(z)\bigr)\;,
%$$
%where $\phe$, $\psi\in\C[\![z]\!]$ are arbitrary power series of order at least~2.

\medbreak
\noindent$\bullet$ {\it Case $(2_{10\rho})$.}

\noindent In this case we have
$$
L(u_{d,j})=(d-j-d\rho+2\rho) u_{d+1,j+1}+(\rho-1)v_{d+1,j}\quad\hbox{and}\quad L(v_{d,j})=(d-j-d\rho+\rho-1)v_{d+1,j+1}
\neweq\eqquno
$$
for all $d\ge 2$ and $j=0,\ldots,d$. Here we can shall see the resonance phenomena we 
mentioned at the beginning of this section: for some values of~$\rho$ the dimension of the kernel of $L|_{\ca H^d}$ can increase, and in some cases
we shall end up with a normal form depending on power series evaluated in monomials
of the form $z^{b-a}w^a$.

Let us put
$$
E_d=\left\{{d-j-1\over d-1}\biggm| j=0,\ldots, d\right\}\setminus\{0\}\quad\hbox{and}\quad
F_d=\left\{{d-j\over d-2}\biggm| j=0,\ldots, d-1\right\}
$$
(we are excluding 0 because $\rho\ne0$ by assumption),
where $E_d$ is defined for all $d\ge 2$ whereas $F_d$ is defined for all $d\ge 3$, and set
$$
\ca E=\bigcup_{d\ge 2} E_d=\bigl((0,1]\cap\Q\bigr)\cup\left\{-{1\over n}\biggm| n\in\N^*\right\}
$$
and
$$
\ca F=\bigcup_{d\ge 3} F_d=\bigl((0,1]\cap\Q\bigr)\cup\left\{1+{1\over n},1+{2\over n}\biggm| n\in\N^*\right\}.
$$
So $\ca E$ is the set of $\rho \in \C^*$ such that $L(v_{d, j})=0$ for some $d\ge 2$ and $0\le j\le d$, while $\ca F$ is the set of $\rho \in \C^*$ such that $L(u_{d, j})=(\rho -1) v_{d+1, j}$ for some $d\ge 3$ and $0\le j\le d-1$. 

\sm
Let us first discuss the non-resonant case, when $\rho\not\in\ca E\cup\ca F$. Then none of the
coefficients in \eqquno\ vanishes, and thus
$$
\Im L|_{\ca H^d}=\Span{(d-d\rho+2\rho) u_{d+1,1} + (\rho -1) v_{d+1,0}, u_{d+1, 2},\ldots,u_{d+1,d+1},v_{d+1,1},\ldots,v_{d+1,d+1}}\;,
$$
and hence
$$
(\Im L|_{\ca H^d})^\perp=\Span{u_{d+1,0},(1-\rho)(d+1)u_{d+1,1} + (d(1-\rho) + 2\rho) v_{d+1,0}}\;.
$$
It then follows that every formal germ of the form
$$
F(z,w)=(z-\rho z^2+O_3,w+(1-\rho)zw+O_3)
$$
with $\rho\not\in\ca E\cup\ca F$ (and $\rho\ne 0$) is formally conjugated to a germ of the form
$$
G(z,w)=\bigl(z-\rho z^2+\phe(w) + (1-\rho) z\psi'(w), w + (1-\rho)zw + (1-\rho) w\psi'(w) + (3\rho -1) \psi(z)\bigr)\;,
$$
where $\phe$,~$\psi\in\C[\![\zeta]\!]$ are arbitrary power series of order at least~3.

Assume now $\rho\in\ca F\setminus\ca E$. Then $L(v_{d,j})\ne O$ always, and thus
$v_{d+1,j}\in\Im L|_{\ca H^d}$ for all $d\ge 2$ and all $j=1,\ldots, d+1$. Since $\rho>1$, if $d>2$ it also follows 
that $u_{d+1,j+1}\in\Im L|_{\ca H^d}$ for $j=1,\ldots,d$. 

Now, if $\rho=1+(1/n)$ then
$$
{d\over d-2}=\rho\quad\Longleftrightarrow\quad d=2(n+1)\;,
$$
and
$$
{d-1\over d-2}=\rho\quad\Longleftrightarrow\quad d=n+2\;.
$$
Taking care of the case $d=2$ separately, we then have
$$
\displaylines{
\Im L|_{\ca H^d}\hfill\cr
=\cases{
\Span{(d-d\rho+2\rho) u_{d+1,1} + (\rho -1) v_{d+1,0}, u_{d+1, 2},\ldots,u_{d+1,d+1},v_{d+1,1},\ldots,v_{d+1,d+1}}\kern-55pt&\cr
&\kern-44pt for $d\ge 3$, $d\ne n+2$, $2(n+1)$,\cr
\Span{u_{d+1,1}+(\rho-1) v_{d+1,0}, u_{d+1,3},\ldots,u_{d+1,d+1},v_{d+1,1},\ldots,v_{d+1,d+1}}&for $d= n+2$,\cr
\Span{u_{d+1,2},\ldots,u_{d+1,d+1},v_{d+1,0},\ldots,v_{d+1,d+1}}&for $d= 2(n+1)$,\cr
\Span{2u_{3,1}+ (\rho -1) v_{3,0},u_{3,2},v_{3,1},v_{3,2},v_{3,3}}&for $d=2$,
\cr}\hfill
\cr}
$$
and hence
$$
\displaylines{
(\Im L|_{\ca H^d}\!)^\perp\hfill\cr
=\cases{
\Span{u_{d+1,0},(1-\rho)(d+1) u_{d+1, 1} + (d(1-\rho)+2\rho)v_{d+1,0}}&for $d\ge 3$, $d\ne n+2$, $2(n+1)$,\cr
\Span{u_{d+1,0},u_{d+1,2},(1-\rho)(d+1)u_{d+1, 1} + v_{d+1, 0}}&for $d= n+2$,\cr
\Span{u_{d+1,0},u_{d+1,1}}&for $d= 2(n+1)$,\cr
\Span{u_{3,0},u_{3,3}, 3(1-\rho)u_{3,1} + 2 v_{3,0}}&for $d=2$.
\cr}\hfill\cr}
%% Note that:
%% if $d= n+2$    then $d(1-\rho) + 2\rho = 1$
%% if $d= 2$      then $d(1-\rho) + 2\rho = 2$
%% if $d= 2(n+2)$ then $d(1-\rho) + 2\rho = 0$
%%
$$
It then follows that every formal germ of the form
$$
F(z,w)=\left(z-\left(1+{1\over n}\right) z^2+O_3,w-{1\over n}zw+O_3\right)
$$
with $n\in\N^*$ is formally conjugated to a germ of the form
$$
\eqalign{
G(z,w)=
&\left(z-\left(1+{1\over n}\right) z^2 + \phe(w) + (1-\rho) z\psi'(w) + a_0 z^3+a_1 z^2 w^{n+1},\right.\cr 
&\quad\left.w-{1\over n}zw + (1-\rho) w\psi'(w) + (3\rho -1) \psi(w)\right)\;,
}
$$
where $\phe$,~$\psi\in\C[\![\zeta]\!]$ are arbitrary power series of order at least~3, and $a_0$, $a_1\in\C$.

If instead $\rho=1+(2/m)$ with $m$ odd (if $m$ is even we are again in the previous case) then 
$$
{d\over d-2}=\rho\quad\Longleftrightarrow\quad d=m+2\;,
$$
whereas ${d-1\over d-2}\ne\rho$ always. Hence
$$
\displaylines{
\Im L|_{\ca H^d}\hfill\cr
=\cases{
\Span{(d-d\rho+2\rho) u_{d+1,1} + (\rho -1) v_{d+1,0},u_{d+1,2},\ldots,u_{d+1,d+1},v_{d+1,1},\ldots,v_{d+1,d+1}}\kern-55pt&\cr
&\kern-30pt for $d\ge 3$, $d\ne m+2$,\cr
\Span{u_{d+1,2},\ldots,u_{d+1,d+1},v_{d+1,0},\ldots,v_{d+1,d+1}}&for $d= m+2$,\cr
\Span{2u_{3,1}+(\rho -1) v_{3,0},u_{3,2},v_{3,1},v_{3,2},v_{3,3}}&for $d=2$,
\cr}\hfill
\cr}
$$
and thus
$$
(\Im L|_{\ca H^d})^\perp=\cases{
\Span{u_{d+1,0},(1-\rho) (d+1)u_{d+1,1} + (d-d\rho+2\rho)  v_{d+1,0}}&for $d\ge 3$, $d\ne m+2$,\cr
\Span{u_{d+1,0},u_{d+1,1}}&for $d= m+2$,\cr
\Span{u_{3,0},u_{3,3},3(1-\rho) u_{3,1} + 2v_{3,0}}&for $d=2$.
\cr}
$$
It then follows that every formal germ of the form
$$
F(z,w)=\left(z-\left(1+{2\over m}\right) z^2+O_3,w-{2\over m}zw+O_3\right)
$$
with $m\in\N^*$ odd is formally conjugated to a germ of the form
$$
\eqalign{
G(z,w)=
&\left(z-\left(1+{2\over m}\right) z^2+\phe(w)+a_0 z^3+ (1-\rho)z(w\psi'(w) + \psi(w)),\right.\cr
&\quad\left.w-{2\over m}zw + (1-\rho) w^2 \psi'(w) + 2\rho w\psi(w)\right)\;,
}
$$
where $\phe\in\C[\![\zeta]\!]$ is an arbitrary power series of order at least~3, $\psi\in\C[\![\zeta]\!]$ is an arbitrary power series of order at least~2, and $a_0$, $a_1\in\C$.

Now let us consider the case $\rho=-1/n\in\ca E\setminus\ca F$. In this case the coefficients
in the expression of $L(u_{d,j})$ are always different from zero (with the exception of $d=j=2$),
whereas 
$$
d-j-d\rho+\rho-1=0\quad\Longleftrightarrow\quad j=d=n+1\;.
$$
It follows that
$$
\displaylines{
\Im L|_{\ca H^d}\hfill\cr
=\cases{
\Span{(d-d\rho+2\rho) u_{d+1,1} + (\rho -1) v_{d+1,0},u_{d+1,2},\ldots,u_{d+1,d+1},v_{d+1,1},\ldots,v_{d+1,d+1}}\kern-57pt&\cr
&for $d\ge 3$, $d\ne n+1$,\cr
\Span{(d-d\rho+2\rho) u_{d+1,1} + (\rho -1) v_{d+1,0},u_{d+1,2},\ldots,u_{d+1,d+1},v_{d+1,1},\ldots,v_{d+1,d}}\kern-57pt&\cr
&for $d= n+1$,\cr
\Span{2u_{3,1}+(\rho-1)v_{3,0},u_{3,2},v_{3,1},v_{3,2},v_{3,3}}&for $d=2$,
\cr}\hfill\cr}
$$
and thus
$$
\displaylines{
(\Im L|_{\ca H^d}\!)^\perp\hfill\cr
=\cases{
\Span{u_{d+1,0},(1-\rho)(d+1)u_{d+1,1} + (d-d\rho+2\rho) v_{d+1,0}}&for $d\ge 3$, $d\ne n+1$,\cr
\Span{u_{d+1,0},v_{d+1,d+1},(1-\rho)(d+1)u_{d+1,1} + (d-d\rho+2\rho) v_{d+1,0}}&for $d= n+1$,\cr
\Span{u_{3,0},u_{3,3},3(1-\rho)u_{3,1} + 2v_{3,0}}&for $d=2$.
\cr}\hfill\cr}
$$
It then follows that every formal germ of the form
$$
F(z,w)=\left(z+{1\over n}z^2+O_3,w+\left(1+{1\over n}\right)zw+O_3\right)
$$
with $n\in\N^*$ is formally conjugated to a germ of the form
$$
\eqalign{
G(z,w)&=\left(z+{1\over n} z^2+\phe(w)+a_0 z^3+(1-\rho)z(w\psi'(w) + \psi(w)),\right.\cr
&\left.\qquad w+\left(1+{1\over n}\right)zw+\psi(z)+a_1z^{n+2} + (1-\rho)w^2\psi'(w) +2\rho w \psi(w) \right)\;,\cr}
$$
where $\phe\in\C[\![\zeta]\!]$ is an arbitrary power series of order at least~3, $\psi\in\C[\![\zeta]\!]$ is an arbitrary power series of order at least~2, and $a_0$, $a_1\in\C$.

Let us now discuss the extreme case
$\rho=1$. It is clear that
$$
\Im L|_{\ca H^d}=\Span{u_{d+1,1},u_{d+1,2},u_{d+1,4},\ldots,u_{d+1,d+1},v_{d+1,2},\ldots,v_{d+1,d+1}}\;,
$$
and hence
$$
(\Im L|_{\ca H^d})^\perp=\Span{u_{d+1,0},u_{d+1,3},v_{d+1,0},v_{d+1,1}}\;,
$$
It then follows that every formal germ of the form
$$
F(z,w)=\left(z-z^2+O_3,w+O_3\right)
$$
is formally conjugated to a germ of the form
$$
G(z,w)=\bigl(z- z^2+\phe_1(w)+z^3\psi(w),
w+\phe_2(w)+z\phe_3(w)\bigr)\;,
$$
where $\phe_1$,~$\phe_2\in\C[\![\zeta]\!]$ are arbitrary power series of order at least~3, $\phe_3\in\C[\![\zeta]\!]$ is an arbitrary power series of order at least~2, and $\psi\in\C[\![\zeta]\!]$ is an arbitrary power series.

We are left with the case $\rho\in(0,1)\cap\Q$. Write $\rho=a/b$ with $a$,~$b\in\N$ coprime and $0<a< b$. Now
$$
d-j-1-{a\over b}(d-1)=0\quad\Longleftrightarrow\quad j={(d-1)(b-a)\over b}\;;
$$
since $a$ and $b$ are coprime, this happens if and only if $d=b\ell+1$ and $j=(b-a)\ell$ for some $\ell\ge 1$. Analogously,
$$
d-j-{a\over b}(d-2)=0\quad\Longleftrightarrow\quad j=d-{a(d-2)\over b}\;;
$$
again, being $a$ and $b$ coprime, this happens if and only if $d=b\ell+2$ and $j=(b-a)\ell+2$ for some $\ell\ge 0$.
It follows that
$$
\displaylines{
\Im L|_{\ca H^d}\hfill\cr
=\cases{
\Span{(d-d\rho+2\rho) u_{d+1,1} + (\rho -1) v_{d+1,0},u_{d+1,2},\ldots,u_{d+1,d+1},v_{d+1,1},\ldots,v_{d+1,d+1}}\kern-60pt&\cr
&\kern-55pt for $d\ge 3$, $d\not\equiv 1$, 2 (mod $b$)\cr
\hbox{\rm Span}\,((d-d\rho+2\rho) u_{d+1,1} + (\rho -1) v_{d+1,0},u_{d+1,2},\ldots,\widehat{u_{d+1,(b-a)\ell+2}},\ldots,u_{d+1,d+1},\kern-60pt&\cr
\kern50pt v_{d+1,1},\ldots,\widehat{v_{d+1,(b-a)\ell+1}},\ldots,v_{d+1,d+1},{a\over b}u_{d+1,(b-a)\ell+2}-\left({a\over b}-1\right)v_{d+1,(b-a)\ell + 1})\kern-60pt&\cr
&for $d=b\ell +1$,\cr
\hbox{\rm Span}\,((d-d\rho+2\rho) u_{d+1,1} + (\rho -1) v_{d+1,0},u_{d+1,2},\ldots,\widehat{u_{d+1,(b-a)\ell+3}},\ldots, u_{d+1,d+1},\kern-60pt&\cr
\kern50pt v_{d+1,1},\ldots,v_{d+1,d+1})&for $d=b\ell+ 2$,\cr
\Span{2u_{3,1}+(\rho-1)v_{3,0},u_{3,2},v_{3,1},v_{3,2},v_{3,3}}&for $d=2$,
\cr}\hfill\cr}
$$
(where the hat indicates that that term is missing from the list), and thus
$$
\displaylines{
(\Im L|_{\ca H^d})^\perp\hfill\cr
=\cases{
\Span{u_{d+1,0},(1-\rho) u_{d+1, 1} + (d-d\rho+2\rho)v_{d+1,0}}&\kern-58pt for $d\ge 3$, $d\not\equiv 1$, 2 (mod $b$),\cr
\hbox{\rm Span}\,(u_{d+1,0},(1-\rho) u_{d+1, 1} + (d-d\rho+2\rho)v_{d+1,0},&\cr
\kern40pt (b-a)(a\ell+1)u_{d+1,(b-a)\ell+2}+a\bigl((b-a)\ell+2\bigr)v_{d+1,(b-a)\ell+1})&for $d=b\ell +1$,\cr
\Span{u_{d+1,0},u_{d+1,(b-a)\ell+3},(1-\rho) u_{d+1, 1} + (d-d\rho+2\rho)v_{d+1,0}}&for $d=b\ell+ 2$,\cr
\Span{u_{3,0},u_{3,3},3(1-\rho) u_{3,1} + 2 v_{3,0}}&for $d=2$.
\cr}\hfill\cr}
$$
It then follows that every formal germ of the form
$$
F(z,w)=\left(z-{a\over b}z^2+O_3,w+\left(1-{a\over b}\right)zw+O_3\right)
$$
with $a/b\in(0,1)\cap\Q$ and $a$, $b$ coprime, is formally conjugated to a germ of the form
$$
\displaylines{
G(z,w)\hfill\cr
=\left(z-{a\over b} z^2+\phe(w)+z^3\phe_0(z^{b-a}w^a)+(b-a){\de\over\de w}\bigl(
z^2w\chi(z^{b-a}w^a)\bigr)+ \left(1-{a\over b}\right) z (w\psi'(w) + \psi(w) \bigr),\right.\cr
\left.\qquad w+\left(1-{a\over b}\right)zw+ a{\de\over\de z}\bigl(z^2w
\chi(z^{b-a}w^a)\bigr)+\left(1-{a\over b}\right) w^2\psi'(w) + 2{a\over b}w\psi(w) \right)\;,\cr}
$$
where $\phe$,~$\psi\in\C[\![\zeta]\!]$ are arbitrary power series of order at least~3, and $\phe_0$,~$\chi\in\C[\![\zeta]\!]$ are arbitrary power series of order at least~1.

%\medbreak
%\noindent$\bullet$ {\it Case $(2_{11\rho})$.}
%
%\noindent In this case we have
%$$
%L(u_{d,j})=-(j\rho+d-j-1)u_{d+1,j}+(d+d\rho-j-2\rho) u_{d+1,j+1}-(1+\rho)v_{d+1,j}
%$$
%and 
%$$
%L(v_{d,j})=-u_{d+1,j+1}+(\rho j-d-j-2)v_{d+1,j}+(d+d\rho-j-1-\rho)v_{d+1,j+1}
%$$
%for all $d\ge 2$ and $j=0,\ldots,d$. ???
%
%\medbreak
%\noindent$\bullet$ {\it Case $(3_{100})$.}
%
%\noindent In this case we have
%$$
%L(u_{d,j})=(1-j)u_{d+1,j}+(j-2)u_{d+1,j+1}\qquad\hbox{and}\qquad L(v_{d,j})=u_{d+1,j+1}+
%j v_{d+1,j+1}-j v_{d+1,j}
%$$
%for all $d\ge 2$ and $j=0,\ldots,d$. It follows that ??? 
%
%\Nota Forse questo si pu\`o fare?
%
%\medbreak
%\noindent$\bullet$ {\it Case $(3_{\rho10})$.}
%
%\noindent In this case we have
%$$
%L(u_{d,j})=\rho(2u_{d+1,j+1}-u_{d+1,j})+(\rho-1)v_{d+1,j}\ \hbox{and}\  
%L(v_{d,j})=-\rho u_{d+1,j+1}+(\rho-1)(v_{d+1,j+1}-2v_{d+1,j})
%\neweq\eqtdue
%$$
%for all $d\ge 2$ and $j=0,\ldots,d$.

%\medbreak
%\noindent$\bullet$ {\it Case $(3_{\rho\tau1})$.}
%
%\noindent In this case we have
%$$
%L(u_{d,j})=(\tau-1)u_{d+1,j}+2\rho u_{d+1,j+1}+(\rho-1)v_{d+1,j}
%$$
%and
%$$  
%L(v_{d,j})=(\tau-1)u_{d+1,j+1}+2\tau v_{d+1,j}+(\rho-1)v_{d+1,j+1}
%$$
%for all $d\ge 2$ and $j=0,\ldots,d$. As before, we have a few subcases to consider.

\bigbreak
\noindent {\bf References.}\setref{AFGG}
\medskip
%\art A M. Abate: The residual index and the dynamics of holomorphic
%maps tangent to the identity! Duke Math. J.! 107 2001 173-207

\art A M. Abate: Holomorphic classification of $2$-dimensional quadratic maps tangent to
the identity! S\=urikaisekiken\-ky\=usho K\=oky\=uroku! 1447 2005 1-14

%\art ABT M. Abate, F. Bracci, F. Tovena: Index theorems for
%holomorphic self-maps!   Ann. of Math.! 159 2004 819-864

\art AT1 M. Abate, F. Tovena: Formal classification of holomorphic maps tangent
to the identity! Disc. Cont. Dyn. Sys.! Suppl. 2005 1-10

\pre AT2 M. Abate, F. Tovena: Poincar\'e-Bendixson theorems for meromorphic connections and homogeneous vector fields! Preprint, arXiv:0903.3485v3! 2009

\art AFGG A. Algaba, E. Freire, E. Gamero. C. Garcia: Quasi-homogeneous normal forms! J. Comput. Appl. Math.! 150 2003 193-216

\book Ar V.I. Arnold: Geometrical methods in the theory of ordinary differential equations! Springer Verlag, New York, 1988

\art B G.R. Belitskii: Invariant normal forms of formal series! Funct. Anal. Appl.! 13 1979 46-67

\art BS A. Baider, J. Sanders: Further reduction of the Takens-Bogdanov normal form! J. Diff. Eq.! 99 1992 205-244

%\art BM F.E. Brochero Mart\'\i nez: Groups of germs of
%analytic diffeomorphisms in $(\C^2,O)$! J. Dynamic. Control Systems! 9
%2003 1-32
%
%\art C C. Camacho: On the local structure of conformal mappings
%and holomorphic vector fields! Ast\'e\-risque! 59--60 1978 83-94

\book Car H. Cartan: Cours de calcul diff\'erentiel, Hermann, Paris! 1977

%\book \'E1 J. \'Ecalle: Les fonctions r\'esurgentes. Tome
%I: Les alg\`ebres de fonctions r\'e\-sur\-gen\-tes! Publ. Math. Orsay {\bf
%81-05,} Universit\'e de Paris-Sud, Orsay, 1981 
%
%\book \'E2 J. \'Ecalle: Les fonctions r\'esurgentes. Tome
%I\negthinspace I: Les fonctions r\'esurgentes appliqu\'ees
%\`a l'it\'eration! Publ. Math. Orsay {\bf 81-06,} Universit\'e de
%Paris-Sud, Orsay, 1981 

\book \'E1 J. \'Ecalle: Les fonctions r\'esurgentes. Tome I\negthinspace
I\negthinspace I: L'\'equation du pont et la classification analytique
des objects locaux! Publ. Math. Orsay {\bf 85-05,} Universit\'e de
Paris-Sud, Orsay, 1985 

\coll \'E2 J. \'Ecalle: Iteration and analytic classification of local
diffeomorphisms of $\C^\nu$! Iteration theory and its
functional equations! Lect. Notes in Math. {\bf 1163,} Springer-Verlag,
Berlin, 1985, pp. 41--48

%\art H M. Hakim: Analytic transformations of $(\C^p,0)$ tangent to the
%identity! Duke Math. J.! 92 1998 403-428
%
%\coll I Yu.S. Il'yashenko: Nonlinear Stokes phenomena! Nonlinear Stokes
%phenomena! Adv. in Soviet Math. {\bf 14,} Am. Math. Soc., Providence,
%1993, pp.~1--55

\art G G. Gaeta: Further reduction of Poincar\'e-Dulac normal forms in symmetric systems! Cubo! 9 2007 1-11

\art KOW H. Kobuki, H. Oka, D. Wang: Linear grading function and further reduction
of normal forms! J. Diff. Eq.! 132 1996 293-318

\pre LS E. Lombardi, L. Stolovitch: Normal forms of analytic perturbations of quasihomogeneous vector fields: Rigidity, analytic invariant sets and exponentially small approximation! Preprint! 2009

%\art M1 B. Malgrange: Travaux d'\'Ecalle et de Martinet-Ramis sur les
%syst\`emes  dynamiques! Ast\'erisque! 92-93 1981/82 59-73
%
%\art M2 B. Malgrange: Introduction aux travaux de J. \'Ecalle! Ens.
%Math.! 31 1985 261-282

\book Mu1 J. Murdock: Normal forms and unfoldings for local dynamical systems! Springer Verlag,
Berlin, 2003

\art Mu2 J. Murdock: Hypernormal form theory: foundations and algorithms! J. Diff. Eq.! 205 2004 424-465

\book R1 J. Raissy: Geometrical methods in the normalization of germs of biholomorphisms! Ph.D. Thesis, Universit\`a di Pisa, 2010

\book R2 J. Raissy: {\sl Brjuno conditions for linearization in presence of resonances}! ArXiv:0911.4341. 
To appear in  {\bf Asymptotics in Dynamics, Geometry and PDE's; Generalized Borel Summation}, Eds. O. Costin, F. Fauvet, F. Menous and D. Sauzin, Edizioni Della Normale, Pisa, 2010

\art R\"u H. R\"ussmann: Stability of elliptic fixed points of analytic area-preserving mappings 
under the Brjuno condition! Ergodic Theory Dynam. Systems! 22 2002 1551-1573

%\art S A.A. Shcherbakov: Topological classification of germs of conformal
%mappings with identity linear part! Moscow Univ. Math. Bull.! 37 1982
%60-65
%
%\art V S.M. Voronin: Analytic classification of germs of conformal maps
%$(\C,0)\to (\C,0)$ with identity linear part! Func. Anal. Appl.! 15 1981
%1-17



\bye
